Revocable Quantum Digital Signatures

We study digital signatures with revocation capabilities and show two results. First, we define and construct digital signatures with revocable signing keys from the LWE assumption. In this primitive, the signing key is a quantum state which enables a user to sign many messages and yet, the quantum key is also revocable, i.e., it can be collapsed into a classical certificate which can later be verified. Once the key is successfully revoked, we require that the initial recipient of the key loses the ability to sign. We construct digital signatures with revocable signing keys from a newly introduced primitive which we call two-tier one-shot signatures, which may be of independent interest. This is a variant of one-shot signatures, where the verification of a signature for the message ``0'' is done publicly, whereas the verification for the message ``1'' is done in private. We give a construction of two-tier one-shot signatures from the LWE assumption. As a complementary result, we also construct digital signatures with quantum revocation from group actions, where the quantum signing key is simply ``returned'' and then verified as part of revocation. Second, we define and construct digital signatures with revocable signatures from OWFs. In this primitive, the signer can produce quantum signatures which can later be revoked. Here, the security property requires that, once revocation is successful, the initial recipient of the signature loses the ability to find accepting inputs to the signature verification algorithm. We construct this primitive using a newly introduced two-tier variant of tokenized signatures. For the construction, we show a new lemma which we call the adaptive hardcore bit property for OWFs, which may enable further applications.

==> 2tierQmoney.tex <==
\section{Two-tier Quantum Money}
\mor{removed later}

\begin{definition}[Two-tier quantum money schemes]
A two-tier quantum money scheme is a set $(\Mint,\SemiVer,\FullVer)$ of algorithms such that
\begin{itemize}
    \item 
    $\Mint(1^\secp)\to(\sk,\pk,\psi_{\sk,\pk}):$
    It is a QPT algorithm that, on input the security parameter $\secp$,
    outputs a classical secret key $\sk$, a classical public key $\pk$, and a quantum money state $\psi_{\sk,\pk}$.
    \item 
    $\FullVer(\sk,\psi)\to\top/\bot:$
    It is a QPT algorithm that, on input $\sk$ and a quantum state $\psi$, outputs $\top/\bot$.
    \item 
    $\SemiVer(\pk,\psi)\to\top/\bot:$
    It is a QPT algorithm that, on input $\pk$ and a quantum state $\psi$, outputs $\top/\bot$.
\end{itemize}
We require the following correctness and security.

\paragraph{Correctness:}
\begin{equation}
\Pr[\top\gets\FullVer(\sk,\psi_{\sk,\pk}):(\sk,\pk,\psi_{\sk,\pk})\gets\Mint(1^\secp)]\ge1-\negl(\secp)    
\end{equation}
and
\begin{equation}
\Pr[\top\gets\SemiVer(\pk,\psi_{\sk,\pk}):(\sk,\pk,\psi_{\sk,\pk})\gets\Mint(1^\secp)]\ge1-\negl(\secp).    
\end{equation}

\paragraph{Security:}
For any QPT adversary $\cA$,
\begin{equation}
\Pr\left[\top\gets\SemiVer(\pk,\psi')\wedge
\top\gets\FullVer(\sk,\psi'')
:
\begin{array}{cc}
(\sk,\pk,\psi_{\sk,\pk})\gets\Mint(1^\secp)\\
(\psi',\psi'')\gets\cA(\pk,\psi_{\sk,\pk})
\end{array}
\right]\le\negl(\secp).    
\end{equation}

\end{definition}

\begin{theorem}
If OWFs exist, then two-tier quantum money schemes exist.
\end{theorem}

\begin{proof}
Let $f$ be a OWF. We construct a two-tier quantum money scheme $(\Mint,\FullVer,\SemiVer)$ as follows.
\begin{itemize}
    \item 
    $\Mint(1^\secp)\to (\sk,\pk,\psi_{\sk,\pk}):$
    Choose $x_i^b\gets\bit^\ell$ for each $b\in\bit$ and $i\in[n]$.
    Output $\sk\coloneqq \{x_i^b\}_{i\in[n],b\in\bit}$,
    $\pk\coloneqq \{f(x_i^b)\}_{i\in[n],b\in\bit}$,
    and $\psi_{\sk,\pk}\coloneqq \bigotimes_{i=1}^n\frac{\ket{x_i^0}+\ket{x_i^1}}{\sqrt{2}}$.
    \item 
    $\FullVer(\sk,\psi)\to\top/\bot:$
    Parse $\sk=\{x_i^b\}_{i,b}$.
    Project $\psi$ onto 
    $\bigotimes_{i=1}^n\frac{\ket{x_i^0}+\ket{x_i^1}}{\sqrt{2}}$.
    If successful, output $\top$. Otherwise, output $\bot$.
        \item 
    $\SemiVer(\pk,\psi)\to\top/\bot:$
    Parse $\pk=\{f(x_i^b)\}_{i,b}$.
    Measure all qubits of $\psi$ in the computational basis to get the result $(z_1,...,z_n)$ with $z_i\in\bit^\ell$.
    If $f(z_i)\in\{f(x_i^0),f(x_i^1)\}$ for all $i\in[n]$, output $\top$.
    Otherwise, output $\bot$.
\end{itemize}
The correctness is clear. Let us show the security.
To show the security, we define the sequence of games, 
Hybrid 0 (\cref{hyb0}), 
Hybrid 1 (\cref{hyb1}).
Hybrid 2 (\cref{hyb2}), and
Hybrid 3 (\cref{hyb3}).
Hybrid 0 is the original security game.
For the sake of contradiction, we
assume that there exists a QPT adversary $\cA$ such that
\begin{align}
\label{assumption}
\Pr[{\rm Hybrid~0}\to\top]\ge\frac{1}{\poly(\secp)}.    
\end{align}

\protocol{Hybrid 0}
{Hybrid 0}
{hyb0}
{
\begin{enumerate}
    \item 
    \label{choosex}
    The challenger $\cC$ chooses $x_i^b\gets\bit^\ell$ for each $i\in[n]$ and $b\in\bit$.
    $\cC$ computes $f(x_i^b)$ for each $i\in[n]$ and $b\in\bit$.
    $\cC$ generates $\bigotimes_{i=1}^n\left(\frac{\ket{x_i^0}+\ket{x_i^1}}{\sqrt{2}}\right)_{\regA_i}$.
    \item 
    $\cC$ sends $\{f(x_i^b)\}_{i,b}$ and
    $\bigotimes_{i=1}^n\left(\frac{\ket{x_i^0}+\ket{x_i^1}}{\sqrt{2}}\right)_{\regA_i}$
    to the adversary $\cA$.
    \item 
    $\cA$ sends a quantum state $\psi_{\regF,\regS}$ over two registers $\regF$ and $\regS$ to $\cC$.
    The register $\regF$ consists of sub-registers $(\regF_1,...,\regF_n)$ and
    the register $\regS$ consists of sub-registers $(\regS_1,...,\regS_n)$.
    Each $\regF_i$ is an $\ell$-qubit register.
    Each $\regS_i$ is an $\ell$-qubit register.
    \item 
    \label{SemiV}
    From $i=1$ to $n$, $\cC$ does the following:
    \begin{enumerate}
        \item 
    Measure the register $\regS_i$ in the computational basis to get the result $z_i\in\bit^\ell$.
    \item
    If $f(z_i)=f(x_i^0)$, set $s_i=0$.
    If $f(z_i)=f(x_i^1)$, set $s_i=1$.
    Otherwise, set $s_i=\bot$.
    \end{enumerate}
    If there is $i\in[n]$ such that $s_i=\bot$, output of the game is $\bot$ and abort.
\item 
    From $i=1$ to $n$, $\cC$ does the following: 
    \begin{enumerate}
        \item 
    Project the register $\regF_i$ onto $\frac{\ket{x_i^0}+\ket{x_i^1}}{\sqrt{2}}$.
    \item
    If successful, set $f_i=1$. Otherwise, set $f_i=0$.
    \end{enumerate}
    \item
    If $f_i=1$ for all $i\in[n]$, the output of the game is $\top$.
    Otherwise, the output of the game is $\bot$.
\end{enumerate}
}


\protocol{Hybrid 1}
{Hybrid 1}
{hyb1}
{
\begin{enumerate}
    \item
    The same as Hybrid 0. 
    \item
    The same as Hybrid 0.
    \item 
    The same as Hybrid 0.
    \item 
    The same as Hybrid 0.
\item 
    From $i=1$ to $n$, $\cC$ does the following: 
    \begin{enumerate}
        \item 
    Measure the register $\regF_i$ in the computational basis to get the result $w_i\in\bit^\ell$.
    \item
    If $w_i=x_i^0$, set $f_i=0$.
    If $w_i=x_i^1$, set $f_i=1$.
    Otherwise, set $f_i=\bot$.
    \end{enumerate}
    If there is $i\in[n]$ such that $f_i=\bot$, the output of the game is $\bot$, and abort.
    \item
    If there is $i\in[n]$ such that $f_i\neq s_i$, the output of the game is $\top$.
    Otherwise, the output of the game is $\bot$.
\end{enumerate}
}


\protocol{Hybrid 2}
{Hybrid 2}
{hyb2}
{
\begin{enumerate}
    \item
    The same as Hybrid 1. 
    \item
    The same as Hybrid 1.
In addition,    
$\cC$ chooses $i^*\gets[n]$.
    \item 
    The same as Hybrid 1.
    \item 
    The same as Hybrid 1.
\item 
The same as Hybrid 1.
\item 
    If $f_{i^*}\neq s_{i^*}$, the output of the game is $\top$.
    Otherwise, the output of the game is $\bot$.
\end{enumerate}
}


\protocol{Hybrid 3}
{Hybrid 3}
{hyb3}
{
\begin{enumerate}
    \item
    The same as Hybrid 2. 
    \item
    $\cC$ chooses $i^*\gets[n]$.
    $\cC$ measures the register $\regA_{i^*}$ in the computational basis.
    Let $\ket{x_{i^*}^d}$ be the post-measurement state, where $d\in\bit$.
        $\cC$ sends $\{f(x_i^b)\}_{i,b}$ and
    $\Big(\bigotimes_{i=1}^{i^*-1}\frac{\ket{x_i^0}+\ket{x_i^1}}{\sqrt{2}}\Big)\otimes
    \ket{x_{i^*}^d}\otimes
    \Big(\bigotimes_{i=i^*+1}^{n}\frac{\ket{x_i^0}+\ket{x_i^1}}{\sqrt{2}}\Big)$
    to the adversary $\cA$.
    \item 
    The same as Hybrid 2.
    \item 
    The same as Hybrid 2.
\item 
The same as Hybrid 2.
\item 
The same as Hybrid 2.
\end{enumerate}
}






\begin{lemma}
\label{lem:01}
If 
$\Pr[{\rm Hybrid~0}\to\top]\ge\frac{1}{\poly(\secp)}$,
then
$\Pr[{\rm Hybrid~1}\to\top]\ge\frac{1}{\poly(\secp)}$.
\end{lemma}

\begin{proof}
For the notational simplicity, define $\mathbf{x}\coloneqq\{x_i^b\}_{i\in[n],b\in\bit}$ and
$\mathbf{s}\coloneqq\{s_i\}_{i\in[n]}$.
Let $p(\mathbf{s}|\mathbf{x})$ be the probability that $\mathbf{s}$ is obtained in \cref{SemiV} of \cref{hyb0}
conditioned that $\mathbf{x}$ is chosen in \cref{choosex} of \cref{hyb0}.
Let $\rho_{\mathbf{x},\mathbf{s}}$ be the state of the register $\regF$ after 
the all operations of \cref{SemiV} of \cref{hyb0} are finished conditioned that $\mathbf{x}$ is chosen in \cref{choosex} of \cref{hyb0}
and $\mathbf{s}$ is obtained in \cref{SemiV} of \cref{hyb0}. 
Define $\Pi_{\mathbf{x}}\coloneqq
\bigotimes_{i=1}^n\frac{\ket{x_i^0}+\ket{x_i^1}}{\sqrt{2}}\frac{\bra{x_i^0}+\bra{x_i^1}}{\sqrt{2}}$.
Then we have
\begin{align}
  \epsilon&\coloneqq \Pr[\mbox{Hybrid 0}\to\top]\\
  &=\frac{1}{2^{2n\ell}}\sum_{\mathbf{x}}
  \sum_{\mathbf{s}\in\bit^n}p(\mathbf{s}|\mathbf{x})
  \Tr\Big[\Pi_{\mathbf{x}}
  \rho_{\mathbf{x},\mathbf{s}}\Big].
\end{align}
From the standard average argument, we have
\begin{align}
\frac{1}{2^{2n\ell}}\sum_{(\mathbf{x},\mathbf{s})\in G}p(\mathbf{s}|\mathbf{x})\ge\frac{\epsilon}{2},    
\label{average}
\end{align}
where
\begin{align}
G\coloneqq\Big\{(\mathbf{x},\mathbf{s}):
  \Tr\Big[\Pi_{\mathbf{x}}\rho_{\mathbf{x},\mathbf{s}}\Big]\ge\frac{\epsilon}{2}
\Big\}.
\label{inG}
\end{align}
Define
$\Lambda_{\mathbf{x},\mathbf{s}}    
\coloneqq
\sum_{\mathbf{s'}\in\bit^n\setminus \{\mathbf{s}\}}
\bigotimes_{i=1}^n\ket{x_i^{s_i'}}\bra{x_i^{s_i'}}$.
Then for any state $\rho$ and any $(\mathbf{x},\mathbf{s})$, we have
 \begin{align}
 \label{PiLambda}
  \Tr\Big[\Pi_{\mathbf{x}} \rho\Big]
  \le
  2\Tr\Big[\Lambda_{\mathbf{x},\mathbf{s}}\rho\Big]+2^{-n+1}. 
\end{align}
This is shown in \cite{cryptoeprint:2023/264}. (For the convenience of readers, we provide the proof in \cref{App:PiLambda}.)
Then we have
\begin{align}
\Pr[\mbox{Hybrid 1}\to\top]&=    
\frac{1}{2^{2n\ell}}\sum_{\mathbf{x}}
\sum_{\mathbf{s}}p(\mathbf{s}|\mathbf{x})\Tr[\Lambda_{\mathbf{x},\mathbf{s}}\rho_{\mathbf{x},\mathbf{s}}]\\
&\ge
\frac{1}{2^{2n\ell}}\sum_{(\mathbf{x},\mathbf{s})\in G}
p(\mathbf{s}|\mathbf{x})\Tr[\Lambda_{\mathbf{x},\mathbf{s}}\rho_{\mathbf{x},\mathbf{s}}]\\
&\ge
\frac{1}{2^{2n\ell}}\sum_{(\mathbf{x},\mathbf{s})\in G}
p(\mathbf{s}|\mathbf{x})\Big[\frac{1}{2}\Tr[\Pi_{\mathbf{x}}\rho_{\mathbf{x},\mathbf{s}}]-2^{-n}\Big]\label{Pinisuru}\\
&\ge\frac{\epsilon}{2}\Big(\frac{\epsilon}{4}-2^{-n}\Big)\label{epsilon}\\
&\ge\frac{1}{\poly(\secp)}.
\end{align}
Here, to derive \cref{Pinisuru}, we have used \cref{PiLambda}.
To derive \cref{epsilon}, we have used \cref{average} and \cref{inG}.
\end{proof}

\begin{lemma}
\label{lem:12}
$\Pr[{\rm Hybrid~2}\to\top]\ge\frac{1}{n}\Pr[{\rm Hybrid~1}\to\top]$.
\end{lemma}
\begin{proof}
It is trivial.
\end{proof}

\begin{lemma}
\label{lem:23}
$\Pr[{\rm Hybrid~3}\to\top]\ge\frac{1}{2}\Pr[{\rm Hybrid~2}\to\top]$.
\end{lemma}
\begin{proof}
   It is clear from \cref{lem:BZ}.
\end{proof}

In summary, from \cref{assumption} and \cref{lem:01,lem:12,lem:23}, we conclude that
$\Pr[{\rm Hybrid~3}\to\top]\ge\frac{1}{\poly(\secp)}$.
From such $\cA$ of Hybrid 3, we construct a QPT adversary $\cB$ that breaks the one-wayness of $f$ as in \cref{cB}.
It is easy to verify that
\begin{align}
\Pr[\cB\to x]&\ge 
\Pr[{\rm Hybrid~3}\to\top]\\
&\ge\frac{1}{\poly(\secp)},
\end{align}
and therefore $\cB$ breaks the one-wayness of $f$.

\protocol{$\cB$}
{$\cB$}
{cB}
{
\begin{enumerate}
    \item 
    Get $f(x)$ as input.
    \item 
    Choose $i^*\gets[n]$.
    Choose $x_i^b\gets\bit^\ell$ for each $i\in[n]\setminus\{i^*\}$ and $b\in\bit$.
    Choose $x'\gets\bit^\ell$.
    Choose $a\gets\bit$.
    Set $y_i^b\coloneqq f(x_i^b)$ for each $i\in[n]\setminus\{i^*\}$ and $b\in\bit$.
    Set $y_{i^*}^a\coloneqq f(x)$ and $y_{i^*}^{a\oplus1}=f(x')$.
    Set $\psi\coloneqq\Big(\bigotimes_{i=1}^{i^*-1}\frac{\ket{x_i^0}+\ket{x_i^1}}{\sqrt{2}}\Big)\otimes\ket{x'}
    \otimes\Big(\bigotimes_{i=i^*+1}^{n}\frac{\ket{x_i^0}+\ket{x_i^1}}{\sqrt{2}}\Big)$.
    \item 
    Run $\rho_{\regF,\regS}\gets \cA(\{y_i^b\}_{i\in[n],b\in\bit},\psi)$.
    \item 
    Measure the register $\regS_{i^*}$ in the computational basis to get the result $z_{i^*}$. 
    Measure the register $\regF_{i^*}$ in the computational basis to get the result $w_{i^*}$. 
    If $f(z_{i^*})=f(x)$, output $z_{i^*}$.
    If $f(w_{i^*})=f(x)$, output $w_{i^*}$.
    Otherwise, output $\bot$.
\end{enumerate}
}




\end{proof}


==> proof_adaptive_hardcore_bit_amp.tex <==
\section{Proof of \cref{thm:adaptive_hardcore_bit_amp}}
\label{sec:proof_adaptive_hardcore_bit_amp}

In this section, we show \cref{thm:adaptive_hardcore_bit_amp}.
For the sake of contradiction,
assume that
there is a QPT algorithm $\mathcal{A}$ such that
\begin{align}
\Pr
\left[
\substack{\forall i \in [n] \,: \, f(x_i) \in \{f(x_i^0),f(x_i^1)\}\ \\
\bigwedge\ \\
\, \forall i \in [n] \,: \, d_i \cdot (x_i^0 \oplus x_i^1) = c_i
}\, \vline \,
\substack{
\forall i \in [n] \,: \, x_i^0\gets\bit^\ell, \, x_i^1\gets\bit^\ell, c_i\gets\bit\\
(\{x_i\}_{i\in[n]},\{d_i\}_{i\in[n]}) \leftarrow \mathcal{A}\left(\bigotimes_{i=1}^n\frac{\ket{x_i^0} +(-1)^{c_i}\ket{x_i^1}}{\sqrt{2}},\{f(x_i^b)\}_{i\in[n],b\in\bit} \right)
}
\right] \ge \frac{1}{\poly(\secp)}
\label{assumption_parallel_hardcorebit_amp}
\end{align}
for infinitely many $\secp$.
From such $\cA$, let us construct the following QPT algorithm $\cB$ for fixed each $(c_1,...,c_n)\in\bit^n$:
\begin{enumerate}
    \item 
    Get $\{f(x_i^b)\}_{i\in[n],b\in\bit}$ and $\bigotimes_{i\in[n]}\frac{\ket{x_i^0}+(-1)^{c_i}\ket{x_i^1}}{\sqrt{2}}$
    as input.
    \item
    Run $(\{x_i\}_{i\in[n]},\{d_i\}_{i\in[n]}) \gets \cA
    \left(\bigotimes_{i=1}^n\frac{\ket{x_i^0} +(-1)^{c_i}\ket{x_i^1}}{\sqrt{2}},\{f(x_i^b)\}_{i\in[n],b\in\bit} \right)
    $.
    \item 
    Output $\{x_i\}_{i\in[n]}$. Set its residual state as $\bigotimes_{i\in[n]}\proj{d_i}$.
\end{enumerate}
Then,
by using the notation of \cref{thm:BKMPW_amp},
we define $\widetilde{\cZ}_\secp^{\cB}(c_1,...,c_n)$.\footnote{Roughly speaking, it is
$\left(\bigotimes_{i\in[n],b\in\bit}\proj{x_i^b}\right)\otimes\left(\bigotimes_{i\in[n]}\proj{d_i}\right)$
if $f(x_i)\in\{f(x_i^0),f(x_i^1)\}$ for all $i\in[n]$,
and it is $\bot$ otherwise.}
Let us consider the following QPT algorithm $\cD$:
\begin{enumerate}
    \item 
    Get $\widetilde{\cZ}_\secp^{\cB}(c_1,...,c_n)$ as input.
    \item 
   If it is $\bot$, output $\bot$.
   Otherwise, parse it as
$\left(\bigotimes_{i\in[n],b\in\bit}\proj{x_i^b}\right)\otimes\left(\bigotimes_{i\in[n]}\proj{d_i}\right)$.
\item 
Compute $c_i'\coloneqq d_i\cdot(x_i^0\oplus x_i^1)$ for each $i\in[n]$.
Output $\{c_i'\}_{i\in[n]}$. 
\end{enumerate}
Then, from \cref{assumption_parallel_hardcorebit_amp},
\begin{align}
\frac{1}{2^n}\sum_{(c_1,...,c_n)\in\bit^n}\Pr[(c_1,...,c_n)\gets\cD(
    \widetilde{\cZ}_\secp^{\cB}(c_1,...,c_n))]\ge\frac{1}{\poly(\secp)}.
    \label{kiketu}
\end{align}
Now we show that it contradicts \cref{thm:BKMPW_amp}.

If \cref{thm:BKMPW_amp} is correct,
\begin{align}
    \left\|
    \widetilde{\cZ}_\secp^{\cB}(c_1,...,c_n)
    -\widetilde{\cZ}_\secp^{\cB}(0,...,0)
    \right\|_1\le\negl(\secp)
\end{align}
for all $(c_1,...,c_n)\in\bit^n$.
However, in that case, 
\begin{align}
\left|
\Pr\left[(c_1,...,c_n)\gets\cD(\widetilde{\cZ}_\secp^{\cB}(c_1,...,c_n))\right]
-\Pr\left[(c_1,...,c_n)\gets\cD(\widetilde{\cZ}_\secp^{\cB}(0,...,0))\right]
\right|
\le\negl(\secp)
\end{align}
for all
$(c_1,...,c_n)\in\bit^n$.
Then from \cref{kiketu}, we have
\begin{align}
\frac{1}{\poly(\secp)}
&\le
\frac{1}{2^n}\sum_{(c_1,...,c_n)\in\bit^n}\Pr[(c_1,...,c_n)\gets\cD(
\widetilde{\cZ}_\secp^{\cB}(c_1,...,c_n))]\\
&\le
\frac{1}{2^n}\sum_{(c_1,...,c_n)\in\bit^n}\Pr[(c_1,...,c_n)\gets\cD(
\widetilde{\cZ}_\secp^{\cB}(0,...,0))]+\negl(\secp)\\
&\le
\frac{1}{2^n}
+\negl(\secp),
\end{align}
which is the contradiction.

    

==> reusable.tex <==
% !TEX root = main.tex
\section{Recyclable Variant}\label{sec:recyclable}
In the construction given in \cref{sec:construction}, a quantum public key can be used to encrypt only one message and a sender needs to obtain a new quantum public key whenever it encrypts a message. This is not desirable from practical perspective. 
In this section, we define recyclable QPKE where a sender only needs to receive one quantum public key to send arbitrarily many messages. The definition is similar to QPKE as defined in~\cref{def:QPKE} except that the encryption algorithm outputs a classical \emph{recycled} key that can be reused to encrypt messages many times.   
%In this section, we show that we can upgrade the scheme into a reusable one where a single quantum public key can be used to encrypt arbitrarily many messages. 

%We define reusable QPKE. The definition is similar to \cite{cryptoeprint:2023/345} with a crucial difference that we allow adversaries to tamper with quantum public keys.

%\takashi{I revised the definition to deal with the issue that an adversary may send a recycled key to the sender.}
\begin{definition}[Recyclable QPKE]
A recyclable QPKE scheme with message space $\bit^\ell$ is a set of algorithms  $(\SKGen,\PKGen,\Enc,\rEnc,\Dec)$ such that
\begin{itemize}
    \item 
    $\SKGen(1^\secp)\to (\sk,\vk):$
    It is a PPT algorithm that, on input the security parameter $\secp$, outputs
    a classical secret key $\sk$ and a classical verification key $\vk$. 
    \item
    $\PKGen(\sk)\to \pk:$
    It is a QPT algorithm that, on input $\sk$, outputs
    a quantum public key $\pk$.
    \item
    $\Enc(\vk,\pk,\msg)\to (\ct,\rk):$ 
    It is a QPT algorithm that, on input $\vk$, $\pk$, and a plaintext $\msg\in\bit^\ell$, outputs a classical ciphertext $\ct$ and classical recycled key $\rk$.  
    \item
    $\rEnc(\rk,\msg)\to \ct:$ 
    It is a PPT algorithm that, on input $\rk$ and a plaintext $\msg\in\bit^\ell$, outputs a classical ciphertext $\ct$. 
    \item
    $\Dec(\sk,\ct)\to \msg':$ 
    It is a classical deterministic polynomial-time algorithm that, on input $\sk$ and $\ct$, outputs $\msg'\in\bit^\ell \cup \{\bot\}$.
\end{itemize}


We require the following correctness and IND-pkTA security.

\paragraph{\bf Correctness:}
 For any $\msg,\msg'\in\bit^\ell$,
\begin{equation}
   \Pr\left[
   \msg\gets\Dec(\sk,\ct)
   \land\\ 
   \msg'\gets\Dec(\sk,\ct'):
   \begin{array}{r}
   (\sk,\vk)\gets\SKGen(1^\secp)\\
   \pk\gets\PKGen(\sk)\\
   (\ct,\rk)\gets\Enc(\vk,\pk,\msg)\\
   \ct'\gets\rEnc(\rk,\msg')
   \end{array}
   \right] \ge 1-\negl(\secp).
\end{equation}

\paragraph{\bf IND-pkTA security under quantum public keys:}
For any polynomial $m$, and any QPT adversary $\cA$,
\begin{equation}
   \Pr\left[b\gets\cA^{\rEnc(\rk,\cdot)}(\ct^\ast ,\st):
   \begin{array}{r}
   (\sk,\vk)\gets\SKGen(1^\secp)\\
   \pk_1,...,\pk_m\gets\PKGen(\sk)^{\otimes m}\\
   (\pk',\msg_0,\msg_1,\st)\gets\cA(\vk,\pk_1,...,\pk_m)\\
   b\gets \bit\\ 
   (\ct^\ast,\rk) \gets\Enc(\vk,\pk',\msg_b)
   \end{array}
   \right] \le \frac{1}{2}+\negl(\secp).
\end{equation}
Here, $\pk_1,...,\pk_m\gets\PKGen(\sk)^{\otimes m}$
means that $\PKGen$ is executed $m$ times and $\pk_i$ is the output of the $i$th execution of $\PKGen$, $\rEnc(\rk,\cdot)$ means a classically-accessible encryption oracle,
and $\st$ is a quantum internal state of $\cA$, which can be entangled with $\pk'$.


\paragraph{\bf IND-pkTA security under recycled keys:} 
For any polynomial $m$, and any QPT adversary $\cA$,
\begin{equation}
   \Pr\left[b\gets\cA^{\rEnc(\rk,\cdot)}(\ct^\ast ,\st'):
   \begin{array}{r}
   (\sk,\vk)\gets\SKGen(1^\secp)\\
   \pk_1,...,\pk_m\gets\PKGen(\sk)^{\otimes m}\\
   (\pk',\msg,\st)\gets\cA(\vk,\pk_1,...,\pk_m)\\
   (\ct,\rk) \gets\Enc(\vk,\pk',\msg)\\
    (\msg_0,\msg_1,\st')\gets \cA^{\rEnc(\rk,\cdot)}(\ct,\st)\\ 
   b\gets \bit\\ 
   \ct^\ast \gets\rEnc(\rk,\msg_b)
   \end{array}
   \right] \le \frac{1}{2}+\negl(\secp).
\end{equation}
Here, $\pk_1,...,\pk_m\gets\PKGen(\sk)^{\otimes m}$
means that $\PKGen$ is executed $m$ times and $\pk_i$ is the output of the $i$th execution of $\PKGen$,  $\rEnc(\rk,\cdot)$ means a classically-accessible encryption oracle, 
and $\st$ and $\st'$ are quantum internal states of $\cA$, which can be entangled with $\pk'$.
%that returns $\rEnc(\rk,\msg)$ on input $\msg$. 
\end{definition}




\iffalse
\begin{definition}[Reusable QPKE]
A reusable QPKE scheme $(\SKGen,\PKGen,\Enc,\Dec)$ with message space $\bit^\ell$ has similar syntax to QPKE as defined in \cref{def:QPKE} except that the encryption algorithm additionally outputs a (possibly quantum) recycled public key in addition to a ciphertext.\footnote{In our construction, recycled public keys are classical.}    
We write $(\ct,\tilde{\pk})\gets \Enc(\msg,\vk,\pk)$ to mean that the encryption algorithm outputs a ciphertext $\ct$ and a recycled key $\tilde{\pk}$. 
We require the following reusable correctness and reusable IND-CPA security.

\paragraph{\bf Reusable correctness:}
For any polynonmial $k$ and $\msg^{(1)},...,\msg^{(k)}\in\bit^\ell$, 
\begin{equation}
   \Pr\left[\msg^{(k)}\gets\Dec(\ct^{(k)},\sk):
   \begin{array}{r}
   (\sk,\vk)\gets\SKGen(1^\secp)\\
   \pk^{(1)}\gets\PKGen(\sk)\\
   \textrm{For~}i=1,2,...,k, (\ct^{(i)},\pk^{(i+1)})\gets\Enc(\vk,\pk^{(i)},\msg^{(i)})\\
   \end{array}
   \right] \ge 1-\negl(\secp).
\end{equation}

\paragraph{\bf Reusable IND-CPA security:}
For any polynomials $m$ and $k$, and any QPT adversary $\cA$, consider the following experiment between $\cA$ and the challenger $\cC$:
\begin{enumerate}
    \item $\cC$ generates $(\sk,\vk)\gets\SKGen(1^\secp)$ and $\pk_1,...,\pk_m\gets\PKGen(\sk)^{\otimes m}$ where $\pk_1,...,\pk_m\gets\PKGen(\sk)^{\otimes m}$
means that $\PKGen$ is executed $m$ times and $\pk_i$ is the output of the $i$th execution of $\PKGen$, and sends $(\vk,\pk_1,...,\pk_m)$ to $\cA$.
\item $\cA$ sends a tampered public key $\pk'$ to $\cC$.
\item $\cC$ lets $\pk^{(1)}:=\pk'$. \takashi{Technically, I could simply say that "$\cA$ sends a tampered public key $\pk^{(1)}$ to $\cA$" in the previous bullet point. Is that better?}\mor{I prefer the current one.}
\item For $i=1,...,k-1$, do the following:
\begin{enumerate}
    \item $\cA$ sends a message $\msg^{(i)}$ to $\cC$.
    \item $\cC$ generates $(\ct^{(i)},\pk^{(i+1)})\gets\Enc(\vk,\pk^{(i)},\msg^{(i)})$ and sends $\ct^{(i)}$ to $\cA$. 
\end{enumerate}
\item $\cA$ sends a challenge message pair $(\msg^{(k)}_0,\msg^{(k)}_1)\in \bit^{\ell\times 2}$ to $\cC$.
\item $\cC$ picks $b\gets \bit$, generates $(\ct^{(k)},\pk^{(k+1)})\gets\Enc(\vk,\pk^{(k)},\msg^{(k)})$ and sends $\ct^{(k)}$ to $\cA$.
\item $\cA$ outputs a bit $b'$.
\end{enumerate}
In the above experiment, we have 
\begin{equation}
   \Pr[b'=b]\le \frac{1}{2}+\negl(\secp).
\end{equation}
\end{definition}
\fi

\paragraph{Construction.} 
We show a generic construction of recyclable QPKE from (non-recyclable) QPKE with classical ciphertexts and IND-CPA secure SKE via standard hybrid encryption.  

Let $\QPKE=(\QPKE.\SKGen,\QPKE.\PKGen,\QPKE.\Enc,\QPKE.\Dec)$ be a (non-recyclable) QPKE scheme with message space $\bit^\secp$ and $\SKE=(\SKE.\Enc,\SKE.\Dec)$ be an SKE scheme with message space $\bit^\ell$. Then we construct a recyclable QPKE scheme $\QPKE'=(\QPKE'.\SKGen,\QPKE'.\PKGen,\QPKE'.\Enc,\allowbreak \QPKE'.\rEnc,\QPKE'.\Dec)$ with message space $\bit^\ell$ as follows:
\begin{itemize}
    \item 
    $\QPKE'.\SKGen(1^\secp)\to (\sk',\vk'):$
    Run  $(\sk,\vk)\gets \QPKE.\SKGen(1^\secp)$ and output a secret key $\sk':=\sk$ and verification key $\vk':=\vk$. 
    \item
    $\QPKE'.\PKGen(\sk')\to \pk':$
    Run $\pk \gets \QPKE.\PKGen(\sk)$ and outputs $\pk':=\pk$. 
    \item
    $\QPKE'.\Enc(\vk',\pk',\msg)\to (\ct',\rk'):$
        Parse $\pk'=\pk$ and $\vk'=\vk$,  
        sample $K\gets \bit^\secp$,  run  $\ct \gets \QPKE.\Enc(\vk,\pk,K)$ and $\ct_{\ske}\gets \SKE.\Enc(K,\msg)$, and output a ciphertext $\ct':=(\ct,\ct_{\ske})$ and recycled key $\rk':=(K,\ct)$.
 \item
 $\QPKE'.\rEnc(\rk',\msg)\to \ct':$
Parse $\rk'=(K,\ct)$, run $\ct_{\ske}\gets \SKE.\Enc(K,\msg)$, and output a ciphertext $\ct':=(\ct,\ct_{\ske})$. 
    \item
    $\QPKE'.\Dec(\sk',\ct')\to \msg':$
    Parse $\ct'=(\ct,\ct_{\ske})$ and $\sk'=\sk$, run $K'\gets \QPKE.\Dec(\sk,\ct)$ and $\msg' \gets \SKE.\Dec(K',\ct_{\ske})$, and output $\msg'$. 
\end{itemize}

\paragraph{Correctness.}
Correctness of $\QPKE'$ immediately follows from correctness of $\QPKE$ and $\SKE$. 

\paragraph{IND-pkTA security.}
IND-pkTA security of $\QPKE$ implies that the SKE key $K$ chosen by $\QPKE'.\Enc$ is computationally indistinguishable from uniformly random for an adversary. Then IND-CPA security of $\SKE$ directly implies IND-pkTA security under quantum public keys and recycled keys of $\QPKE'$ 
since $\msg$ is encrypted by $\SKE$ under the key $K$ in both of  $\QPKE'.\Enc$ and $\QPKE'.\rEnc$. 
%When $k\geq 2$, the challenge message pair will be encrypted under a recycled public key $\tilde{\pk}=(1,K,\ct)$ where $K$ is computationally indistinguishable from uniformly random as

\begin{remark}
We can generically add decryption error detectability by using digital signatures similarly to (non-recyclable) QPKE. 
\end{remark}

==> revQsig.tex <==
\section{Signature-Revocable Quantum Digital Signatures}

\begin{definition}[Signature-revocable quantum digital signatures]
Signature-revocable quantum digital signatures is a set $(\Gen,\Sign,\Ver,\Rev)$ of algorithms such that
\begin{itemize}
    \item 
    $\Gen(1^\secp)\to(\sk,\pk):$
    It is a QPT algorithm that, on input the security parameter $\secp$, outputs a classical secret key $\sk$ and a classical public key $\pk$.
    \item 
    $\Sign(\sk,m)\to\sigma:$
    It is a QPT algorithm that, on input $\sk$ and a message $m$, outputs a quantum signature $\sigma$.
    \item 
    $\Ver(\pk,\rho)\to\top/\bot:$
    It is a QPT algorithm that, on input $\pk$ and a quantum state $\rho$, outputs $\top/\bot$.
    \item 
    $\Rev(\sk,\rho)\to\top/\bot:$
    It is a QPT algorithm that, on input $\sk$ and a quantum state $\rho$, outputs $\top/\bot$.
\end{itemize}
We require the following correctness, one-time security, and revocability.

\paragraph{Correctness:}
For any $m$,
\begin{equation}
\Pr[\top\gets\Ver(\pk,m,\sigma):(\sk,\pk)\gets\Gen(1^\secp),\sigma\gets\Sign(\sk,m)]\ge1-\negl(\secp).    
\end{equation}

\paragraph{One-time security:}
For any QPT adversary $\cA$,
\begin{equation}
\Pr[\top\gets\Ver(\pk,m,\sigma):(\sk,\pk)\gets\Gen(1^\secp),(\sigma,m)\gets\A(\pk)]\le\negl(\secp).    
\end{equation}
\mor{Can we make this many-time secure?}
\takashi{I think there is a simple compiler that upgrades one-time security to many-time security as follows. 
The key generation algorithm generates sk and pk of a (not necessarily revocable) many-time secure signature scheme.
Whenever generating a signature, the signer generates a fresh sk and pk of the one-time scheme, use the sk of the one-time scheme to generate a signature on the message and use the sk of the many-time secure scheme to generate a signature on the pk of the one-time scheme.}

\paragraph{Revocability:}
For any QPT adversary $\cA$ and for any $m$,
\begin{equation}
\Pr\left[\top\gets\Ver(\pk,m,\sigma')\wedge
\top\gets\Rev(\sk,\sigma'')
:
\begin{array}{cc}
(\sk,\pk)\gets\Gen(1^\secp)\\
\sigma\gets\Sign(\sk,m)\\
(\sigma',\sigma'',m)\gets\cA(\pk,\sigma)
\end{array}
\right]\le\negl(\secp).    
\end{equation}
\takashi{Note that we can achieve "many-time revocability" where the adversary gets many signatures by the above conversion.}
\end{definition}

\begin{theorem}
If OWFs exist then signature-revocable quantum digital signatures exist.    
\end{theorem}

\begin{proof}
Let $f$ be a OWF.    
From it, we construct signature-revocable quantum digital signatures $(\Gen,\Sign,\Ver,\Rev)$
as follows:
\begin{itemize}
    \item 
    $\Gen(1^\secp)\to(\sk,\pk):$
    Choose $x_i^b(m)\gets\bit^\ell$ for each $i\in[n]$, $b\in\bit$, and $m\in\bit$.
    Choose $c_i(m)\gets\bit$ for each $i\in[n]$ and $m\in\bit$.
    Output $\sk\coloneqq (\{x_i^b(m)\}_{i,b,m},\{c_i(m)\}_{i,m})$ and
    $\pk\coloneqq \{f(x_i^b(m))\}_{i,b,m}$.
    \item 
    $\Sign(\sk,m)\to\sigma:$
    Parse $\sk=(\{x_i^b(m)\}_{i,b,m},\{c_i(m)\}_{i,m})$.
    Output $\sigma \coloneqq\bigotimes_i \frac{\ket{x_i^0(m)}+(-1)^{c_i(m)}\ket{x_i^1(m)}}{\sqrt{2}}$.
    \item 
    $\Ver(\pk,m,\sigma)\to\top/\bot:$
    Parse $\pk=\{f(x_i^b(m))\}_{i,b,m}$.
    Parse $\sigma=\bigotimes_i \frac{\ket{x_i^0(m)}+(-1)^{c_i(m)}\ket{x_i^1(m)}}{\sqrt{2}}$.
    Measure $\sigma$ in the computational basis to get the result $\{z_i\}_i$, where
    $z_i\in\bit^\ell$ for each $i\in[n]$.
    If $f(z_i)\in\{f(x_i^0(m)),f(x_i^1(m))\}$ for all $i\in[n]$, output $\top$. 
    Otherwise, output $\bot$.
    \item 
    $\Rev(\sk,m,\sigma)\to\top/\bot:$
    Parse $\sk=(\{x_i^b(m)\}_{i,b,m},\{c_i(m)\}_{i,m})$.
    Parse $\sigma=\bigotimes_i \frac{\ket{x_i^0(m)}+(-1)^{c_i(m)}\ket{x_i^1(m)}}{\sqrt{2}}$.
    Measure $\sigma$ in the Hadamard basis to get the result $\{d_i\}_i$.
    If $d_i\cdot (x_i^0(m)\oplus x_i^1(m))=c_i(m)$ for all $i\in[n]$, output $\top$.
    Otherwise, output $\bot$.
\end{itemize}
The correctness is clear. The security is also straightforwardly reduced to the (amplified version of) adaptive hardcore bit
property for OWFs \cref{thm:adaptive_hardcore_bit_amp}.
\end{proof}
    

==> revocableQM.tex <==
\section{Revocable Public-Key Quantum Money}
\label{sec:revocable_money}

In this section, we define a new primitive which we call revocable (public-key) quantum money ($\mathsf{RQM}$). Informally, this is a (public-key) quantum money scheme which has an additional feature that allows the bank\mor{only bank?} to \emph{revoke} quantum banknotes. Here, the security property ensures that, once revocation is successful, the initial recipient of the quantum banknote no longer has the ability to find accepting inputs to the (public) money verification algorithm. As mentioned in the introduction, this new primitive naturally gives rise to revocable quantum trust funds. Let us now give a formal definition.

\subsection{Definition}

\begin{definition}[Revocable Public-Key Quantum Money]

Let $\lambda \in \N$ be the security parameter. A revocable public-key quantum money scheme $(\mathsf{RQM})$ is a tuple of QPT algorithms $(\KeyGen,\Bank,\Ver,\Del,\Cert)$:
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to (\sk,\pk):$
    It is a QPT algorithm that, on input the security parameter $\secp$, outputs a classical secret key $\sk$ and
    a classical public key $\pk$. 
    \item 
    $\Bank(\sk)\to (\ck,\$):$
    It is a QPT algorithm that, on input the secret key $\sk$, generates a classical certification key $\ck$ and a quantum banknote $\$ = (s,\rho_s)$ consisting of a classical serial number $s$ and associated quantum money state $\rho_s$.
    \item 
    $\Ver(\pk,\sigma)\to\top/\bot:$
    It is a QPT algorithm that, on input the public key $\pk$ and an alleged quantum banknote $\sigma$, outputs $\top/\bot$.
    \item 
    $\Del(\$)\to\cert:$
    It is a QPT algorithm that, on input a quantum banknote $\$$, outputs a classical certificate $\cert$.
    \item 
    $\Cert(\ck,\cert)\to\top/\bot:$
    It is a QPT algorithm that, on input $\ck$ and $\cert$, outputs $\top/\bot$.
\end{itemize}
We require the following properties.

\paragraph{Correctness:}
For all $\lambda \in \N$, it holds that
\begin{align}
\Pr
\left[\top\gets\Ver(\pk,\$):
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
(\$,\ck)\gets\Bank(\sk)
\end{array}
\right]
\ge1-\negl(\secp).
\end{align}


\paragraph{Deletion correctness:}
For all $\lambda \in \N$, it holds that
\begin{align}
   \Pr\left[
   \top\gets\Cert(\ck,\cert):
   \begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
(\$,\ck)\gets\Bank(\sk)\\
   \cert\gets\Del(\$)
  \end{array}
  \right] 
   \ge1-\negl(\secp).
\end{align}


\paragraph{Unforgeability:}

For all $\lambda \in \N$ and for any QPT counterfeiter $\cA$, which maps $q=\poly(\lambda)$ valid banknotes to $r=\poly(\lambda)$ many (possibly entangled) alleged banknotes, it holds that
\begin{align}
   \Pr\left[
   \mathsf{Count}(\pk,\cA(\pk,\$_1,\dots,\$_q))>q:
   \begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
(\$_1,\ck_1)\gets\Bank(\sk)\\
\vdots \phantom{quad}\\
(\$_q,\ck_q)\gets\Bank(\sk)
  \end{array}
  \right] 
   \le \negl(\secp),
\end{align}
where $\mathsf{Count}(\pk,\psi_1,\dots,\psi_r)$ takes as input the public key $\pk$ and a number of (possibly entangled) alleged banknotes $(\psi_1,\dots,\psi_r)$, and outputs the number of indices $i\in[r]$ such that $\Ver(\pk,\psi_i) = \top$.

\paragraph{Deletion security:}
For any QPT adversary $\cA$,
\begin{align}
\Pr\left[\top\gets\Cert(\ck,\cert)\wedge \top\gets\Ver(\pk,\$^*):
   \begin{array}{rr}
   (\sk,\pk)\gets\KeyGen(1^\secp)\\
    (\$,\ck)\gets\Bank(\sk)\\
    (\cert,\$^*)\gets\cA(\$,\pk)\\
   \end{array}
   \right] 
   \le\negl(\secp).
   \label{money-deletionsecurity}
\end{align}
\alex{This is may not be the ideal definition yet. Maybe we should give $\cA$ many banknotes and ask to delete them all? This means that in Theorem 8.2 we probably need a DSR-Sign scheme which has a slightly stronger many-time deletion guarantee where we also hand out many quantum signatures on $m^*$ and ask to delete them all, as in Remark 7.2?}\mor{I think so, because $\$$ is rather ``coin". However, if there is no time, maybe the current weak version is OK as a first toy example.}
\end{definition}

\subsection{Construction}

In this section, we prove the following theorem.

\begin{theorem}
Revocable public-key quantum money schemes exist if  both mini-schemes and digital signature schemes
with revocable signatures exist.
\end{theorem}

\begin{proof}
Let $\mathcal{M}=(\Bank,\Ver)$ be a mini-scheme and 
$\Sigma=(\KeyGen,\Sign,\Ver,\Del,\Cert)$ be a digital signature scheme
with revocable signatures. We consider the following scheme $\mathsf{RQM}=(\KeyGen,\Bank,\Ver,\Del,\Cert)$:
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to (\sk,\pk):$
    run $(\sigk,\vk) \leftarrow \Sigma.\KeyGen(1^\lambda)$ and output $\sk:=\sigk$ and $\pk:=\vk$.
    \item 
    $\Bank(\sk)\to (\ck,\$):$
    run $(s,\rho_s) \gets \mathcal{M}.\Bank(1^\lambda)$ and generate $(\psi,\ck') \gets \Sigma.\Sign(\sk,s)$, and output the quantum banknote $\$ = (s,\psi,\rho_s)$ and the certification key $\ck := \ck'$.
    \item 
    $\Ver(\pk,\$)\to\top/\bot:$
    on input an alleged banknote $\$ = (s,\psi,\rho)$, output $\top$ if $\mathcal{M}.\Ver(s,\rho) = \top$ and $\Sigma.\Ver(\pk,\psi,s) = \top$, and output $\bot$ otherwise.
    \item 
    $\Del(\$)\to\cert:$
    on input $\$ = (s,\psi,\rho)$, output the classical certificate $\cert \gets \Sigma.\Del(\psi)$.
    \item 
    $\Cert(\ck,\cert)\to\top/\bot:$
    on input $(\ck,\cert)$, output whatever $\Sigma.\Cert(\ck,\cert)$ outputs.
\end{itemize}
Note that correctness and deletion correctness of $\mathsf{RQM}$ follow immediately from the relevant properties of the underlying schemes $\mathcal{M}$ and $\Sigma$. The proof of unforgeability is virtually identical to \cite[Theorem 16]{AC12}.

We now show that $\mathsf{RQM}$ satisfies deletion security. Suppose for the sake of contradiction that there exists a QPT adversary $\cA$ and a polynomial $p(\lambda)$ such that for infinitely many $\lambda \in \N$:
\begin{align}
\Pr\left[\top\gets\Cert(\ck,\cert)\wedge \top\gets\Ver(\pk,\psi):
   \begin{array}{rr}
   (\sk,\pk)\gets\KeyGen(1^\secp)\\
    (\$,\ck)\gets\Bank(\sk)\\
    (\cert,\psi)\gets\cA(\$,\pk)\\
   \end{array}
   \right] 
   \ge \frac{1}{p(\secp)}.
   \label{money-deletionsecurity-adv}
\end{align}
We now show that we can use the adversary $\cA$ which satisfies \eqref{money-deletionsecurity-adv} to break the many-time deletion security of the scheme $\Sigma$. Consider the following reduction:
\begin{enumerate}
    \item On input $\vk$, where $(\sigk,\vk) \gets \Sigma.\KeyGen(1^\lambda)$, run $(s,\rho_s) \gets \mathcal{M}.\Bank(1^\lambda)$ and submit the query $s$ to the signing oracle $\Sigma.\Sign(\sigk,\cdot)$ to receive $(\psi,\ck)$.

    \item Generate the quantum banknote $\$ = (s,\psi,\rho_s)$ and send $\$$ to $\cA$. 
    
    \item When $\cA$ replies with $(\cert,\$^*)$, parse $\$^* = (s^*,\psi^*,\rho^*)$ and output $(\cert,\psi^*)$.
    \end{enumerate}
Note that \eqref{money-deletionsecurity-adv} implies that both $\Sigma.\Cert(\ck,\cert)$ and $\Sigma.\Ver(\vk,\psi^*)$ output $\top$ with probability at least $1/p(\lambda)$. This breaks the many-time deletion security of $\Sigma$. This proves the claim.
\end{proof}


==> skrevoke.tex <==
\section{Digital Signatures with Revocable Signing Keys}
\label{sec:skrevoke}
\mor{I will write later.}
\subsection{Definition}
\begin{definition}
\end{definition}

\subsection{Construction}
It can be constructed from two-tier quantum lightning in a black-box way.
\mor{Because two-tier quantum lightning can be constructed from GA but two-tier one-shot signature does not seem to be so,
it is meaningful to define and construct digital signatures with revocable signing keys.}

==> twotierprimitives.tex <==
\section{Two-tier primitives}
\label{Sec:twotierprimitives}

In this section, we define four primitives, two-tier quantum money,
two-tier quantum lightning, two-tier quantum tokenized signatures,
and two-tier quantum one-shot signatures.
Two-tier quantum lightning was introduced in \cite{TCC:KitNisYam21}.
Other three primitives are newly introduced here.
We also show the constructions of them.

\subsection{Definitions}
In this subsection, we define these four primitives.

\subsubsection{Two-tier quantum money}
\mor{Will we use it?}
We first define two-tier quantum money. (Publicly-verifiable) quantum money is a primitive where
no QPT adversary who receives a single copy of a money state can output two copies of money states that are
both accepted by the public verification algorithm.
Two-tier quantum money is its variant where the security is slightly modified as follows:
no QPT adversary who receives a single copy of a money state can output two copies of money states 
one of which is accepted by a public verification algorithm
and the other of which is accepted by a {\it private} verification algorithm.
Its formal definition is given as follows.
\begin{definition}[Two-tier quantum money]
Two-tier quantum money is a set \break $(\KeyGen,\StateGen,\SemiVer,\FullVer)$
of algorithms such that
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to(\sk,\pk):$
    It is a QPT algorithm that, on input the security parameter $\secp$, outputs
    a classical secret key $\sk$ and a classical public key $\pk$.
    \item 
    $\StateGen(\sk)\to\psi:$
    It is a QPT algorithm that, on input $\sk$, outputs 
    a quantum state $\psi$.
    \item 
    $\SemiVer(\pk,\psi)\to\top/\bot:$
    It is a QPT algorithm that, on input $\pk$ and $\psi$, outputs $\top/\bot$.
    \item 
    $\FullVer(\sk,\psi)\to\top/\bot:$
    It is a QPT algorithm that, on input $\sk$ and $\psi$, outputs $\top/\bot$.
\end{itemize}
We require the following properties.

\paragraph{Correctness:}
\begin{align}
\Pr\left[\top\gets\SemiVer(\pk,\psi):
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
\psi\gets\StateGen(\sk)\\
\end{array}
\right]\ge1-\negl(\secp)    
\end{align}
and
\begin{align}
\Pr\left[\top\gets\FullVer(\sk,\psi):
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
\psi\gets\StateGen(\sk)\\
\end{array}
\right]\ge1-\negl(\secp).
\end{align}

\paragraph{Security:}
For any QPT adversary $\cA$,
\begin{align}
\Pr\left[
\top\gets\SemiVer(\pk,\sigma_0)
\wedge
\top\gets\FullVer(\sk,\sigma_1)
:
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
\psi\gets\StateGen(\sk)\\
(\sigma_0,\sigma_1)\gets\cA(\psi,\pk)\\
\end{array}
\right]\le\negl(\secp).    
\end{align}
\end{definition}


\subsubsection{Two-tier quantum lightning}
Two-tier quantum lightning was introduced in \cite{TCC:KitNisYam21}.
It is a variant of quantum lightning introduced in \cite{JC:Zhandry21}.
The main difference of quantum lightning from (publicly-verifiable) quantum money
is that the security is guaranteed even if money states are generated by the adversary.
The formal definition of two-tier quantum lightning is given as follows.
\begin{definition}[Two-tier quantum lightning \cite{TCC:KitNisYam21}]
Two-tier quantum lighting is a set \break $(\KeyGen,\StateGen,\SemiVer,\FullVer)$
of algorithms such that
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to(\sk,\pk):$
    It is a QPT algorithm that, on input the security parameter $\secp$, outputs
    a classical secret key $\sk$ and a classical public key $\pk$.
    \item 
    $\StateGen(\pk)\to(\psi,\snum):$
    It is a QPT algorithm that, on input $\pk$, outputs 
    a quantum state $\psi$ and a classical serial number $\snum$.
    \item 
    $\SemiVer(\pk,\psi,\snum)\to\top/\bot:$
    It is a QPT algorithm that, on input $\pk$, $\psi$, and $\snum$, outputs $\top/\bot$.
    \item 
    $\FullVer(\sk,\psi,\snum)\to\top/\bot:$
    It is a QPT algorithm that, on input $\sk$, $\psi$, and $\snum$, outputs $\top/\bot$.
\end{itemize}
We require the following properties.

\paragraph{Correctness:}
\begin{align}
\Pr\left[\top\gets\SemiVer(\pk,\psi,\snum):
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
(\psi,\snum)\gets\StateGen(\pk)\\
\end{array}
\right]\ge1-\negl(\secp)    
\end{align}
and
\begin{align}
\Pr\left[\top\gets\FullVer(\sk,\psi,\snum):
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
(\psi,\snum)\gets\StateGen(\pk)\\
\end{array}
\right]\ge1-\negl(\secp).
\end{align}

\paragraph{Security:}
For any QPT adversary $\cA$,
\begin{align}
\Pr\left[
\top\gets\SemiVer(\pk,\psi_0,\snum)
\wedge
\top\gets\FullVer(\sk,\psi_1,\snum)
:
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
(\psi_0,\psi_1,\snum)\gets\cA(\pk)\\
\end{array}
\right]\le\negl(\secp).    
\end{align}
\end{definition}

\begin{remark}
In the definition in \cite{TCC:KitNisYam21}, $\SemiVer$ also outputs a quantum state $\psi'$,
but in this paper, we consider a simpler syntax where
$\SemiVer$ outputs only $\top/\bot$.
\end{remark}


\subsubsection{Two-tier tokenized signatures}
Tokenized signatures was introduced in \cite{BenDavidSattath}. 
The main difference of tokenized signatures from (publicly verifiable) quantum money is the following:
In quantum money, no QPT adversary can output two quantum states (money states) both of which are accepted by the public verification algorithm.
In tokenized signatures, on the other hand, no QPT adversary can output two classical bit strings (signatures) both of which are accepted by the public verification algorithm.

Here, we introduce a variant of tokenized signatures that we call two-tier tokenized signatures.
Intuitively, it is tokenized signatures for a single-bit message with two verification algorithms for signatures.
One algorithm $\Ver_0$ is the verification algorithm for message 0, and it uses the public key.
The other algorithm $\Ver_1$ is the verification algorithm for message 1, and it uses the {\it secret} key.
The formal definition is as follows.

\begin{definition}[Two-tier tokenized signatures]
Two-tier tokenized signature is a set \break $(\KeyGen,\StateGen,\Sign,\Ver_0,\Ver_1)$ of algorithms such that
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to (\sk,\pk):$
    It is a QPT algorithm that, on input the security parameter $\secp$, outputs
    a classical secret key $\sk$ and a classical public key $\pk$.
    \item 
    $\StateGen(\sk)\to\psi:$
    It is a QPT algorithm that, on input $\sk$, outputs a quantum state $\psi$.
    \item 
    $\Sign(\psi,m)\to\sigma:$
    It is a QPT algorithm that, on input $\psi$ and a message $m\in\bit$, outputs a classical signature $\sigma$.
    \item 
    $\Ver_0(\pk,\sigma)\to\top/\bot:$
    It is a QPT algorithm that, on input $\pk$ and $\sigma$, outputs $\top/\bot$.
    \item 
    $\Ver_1(\sk,\sigma)\to\top/\bot:$
    It is a QPT algorithm that, on input $\sk$ and $\sigma$, outputs $\top/\bot$.
\end{itemize}
We require the following properties.

\paragraph{Correctness:}
\begin{align}
\Pr\left[\top\gets\Ver_0(\pk,\sigma):
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
\psi\gets\StateGen(\sk)\\
\sigma\gets\Sign(\psi,0)
\end{array}
\right]\ge1-\negl(\secp)    
\end{align}
and
\begin{align}
\Pr\left[\top\gets\Ver_1(\sk,\sigma):
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
\psi\gets\StateGen(\sk)\\
\sigma\gets\Sign(\psi,1)
\end{array}
\right]\ge1-\negl(\secp).
\end{align}


\paragraph{Security:}
For any QPT adversary $\cA$,
\begin{align}
\Pr\left[
\top\gets\Ver_0(\pk,\sigma_0)
\wedge
\top\gets\Ver_1(\sk,\sigma_1)
:
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
\psi\gets\StateGen(\sk)\\
(\sigma_0,\sigma_1)\gets\cA(\psi,\pk)
\end{array}
\right]\le\negl(\secp).
\end{align}
\end{definition}

We can show that the following type of security, which we call {\it one-wayness}, is also satisfied by
two-tier tokenized signatures.
\begin{lemma}[One-wayness of two-tier tokenized signatures]
\label{lem:onewayness}
For any QPT adversary $\cA$,
\begin{align}
\Pr\left[
\top\gets\Ver_0(\pk,\sigma)
:
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
\psi\gets\cA(\pk)\\
\sigma\gets\Sign(\psi,0)
\end{array}
\right]\le\negl(\secp).
\end{align}
\end{lemma}

\begin{proof}
Assume that there exists a QPT adversary $\cA$ such that
\begin{align}
\Pr\left[
\top\gets\Ver_0(\pk,\sigma)
:
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
\psi\gets\cA(\pk)\\
\sigma\gets\Sign(\psi,0)
\end{array}
\right]\ge\frac{1}{\poly(\secp)}.
\end{align}
Then, from such $\cA$, we can construct a QPT adversary $\cB$ that breaks two-tier tokenized signatures as follows:
\begin{enumerate}
    \item 
    Get $\psi$ and $\pk$ as input.
    \item 
    Run $\psi'\gets\cA(\pk)$.
    \item 
    Run $\sigma_0\gets\Sign(\psi',0)$ and
    $\sigma_1\gets\Sign(\psi,1)$.
    \item 
    Output $(\sigma_0,\sigma_1)$.
\end{enumerate}
It is clear that $\cB$ breaks two-tier tokenized signatures.
\end{proof}



\subsubsection{Two-tier one-shot signatures}
One-shot signatures was introduced in \cite{STOC:AGKZ20}.
The main difference of one-shot signatures from tokenized signatures is that the security is guaranteed even if
the quantum state is generated by the adversary.

We here introduce a variant of one-shot signatures, which we call two-tier one-shot signatures.
The main difference from one-shot signatures is that there are two verification algorithms, and the signature for message 0 is verified by a public verification algorithm,
while the signature for massage 1 is verified by a {\it private} verification algorithm.
Its formal definition is as follows.

\begin{definition}[Two-tier one-shot signatures]
Two-tier one-shot signatures is a set \break $(\Setup,\KeyGen,\Sign,\Ver_0,\Ver_1)$ of algorithms such that
\begin{itemize}
\item 
$\Setup(1^\secp)\to(\pp,\sk):$
It is a QPT algorithm that, on input the security parameter $\secp$, outputs a classical parameter $\pp$ and a classical secret key $\sk$.
    \item 
    $\KeyGen(\pp)\to (\sigk,\vk):$
    It is a QPT algorithm that, on input $\pp$, outputs
    a quantum signing key $\sigk$ and a classical verification key $\vk$.

%    \item 
%    $\StateGen(\pk)\to\psi:$
%    It is a QPT algorithm that, on input $\pk$, outputs a quantum state $\psi$.
    \item 
    $\Sign(\sigk,m)\to\sigma:$
    It is a QPT algorithm that, on input $\sigk$ and a message $m\in\bit$, outputs a classical signature $\sigma$.
    \item 
    $\Ver_0(\pp,\vk,\sigma)\to\top/\bot:$
    It is a QPT algorithm that, on input $\pp$, $\vk$, and $\sigma$, outputs $\top/\bot$.
    \item 
    $\Ver_1(\pp,\sk,\sigma)\to\top/\bot:$
    It is a QPT algorithm that, on input $\pp$, $\sk$, and $\sigma$, outputs $\top/\bot$.
\end{itemize}
\mor{I have changed the syntax. It will be further changed later, so that it fits the revocable signing key digital signature.}
We require the following properties.

\paragraph{Correctness:}
\begin{align}
\Pr\left[
\top\gets\Ver_0(\pp,\vk,\sigma):
\begin{array}{rr}
(\sk,\pp)\gets\Setup(1^\secp)\\
(\sigk,\vk)\gets\KeyGen(\pp)\\
\sigma\gets\Sign(\sigk,0)
\end{array}
\right]\ge1-\negl(\secp)    
\end{align}
and
\begin{align}
\Pr\left[\top\gets\Ver_1(\pp,\sk,\sigma):
\begin{array}{rr}
(\sk,\pp)\gets\Setup(1^\secp)\\
(\sigk,\vk)\gets\KeyGen(\pp)\\
\sigma\gets\Sign(\sigk,1)
\end{array}
\right]\ge1-\negl(\secp).
\end{align}


\paragraph{Security:}
For any QPT adversary $\cA$,
\begin{align}
\Pr\left[
\top\gets\Ver_0(\pp,\vk,\sigma_0)
\wedge
\top\gets\Ver_1(\pp,\sk,\sigma_1)
:
\begin{array}{rr}
(\sk,\pp)\gets\Setup(1^\secp)\\
(\vk,\sigma_0,\sigma_1)\gets\cA(\pp)
\end{array}
\right]\le\negl(\secp).
\end{align}
\end{definition}




\subsection{Constructions}
In this subsection, we
provide constructions of these four primitives.

\subsubsection{Two-tier tokenized signatures}
We first show that two-tier tokenized signatures can be constructed from OWFs.
\begin{theorem}
If OWFs exist, then two-tier tokenized signatures exist.
\end{theorem}

\begin{proof}
   Let $f$ be a OWF. From it, we construct a two-tier tokenized signature as follows:
\begin{itemize}
     \item 
    $\KeyGen(1^\secp)\to (\sk,\pk):$
    Choose $x_i^0,x_i^1\gets\bit^\ell$ for each $i\in[n]$.
    Choose $c_i\gets\bit$ for each $i\in[n]$.
    Output $\sk\coloneqq\{c_i,x_i^0,x_i^1\}_{i\in[n]}$
    and $\pk\coloneqq\{f(x_i^0),f(x_i^1)\}_{i\in[n]}$.
    \item 
    $\StateGen(\sk)\to\psi:$
    Parse $\sk=\{c_i,x_i^0,x_i^1\}_{i\in[n]}$.
    Output $\psi\coloneqq\bigotimes_{i\in[n]}\frac{\ket{x_i^0}+(-1)^{c_i}\ket{x_i^1}}{\sqrt{2}}$. 
    \item 
    $\Sign(\psi,m)\to\sigma:$
    If $m=0$, measure $\psi$ in the computational basis to get the result $\{z_i\}_{i\in[n]}$ (where $z_i\in\bit^\ell$ for each $i\in[n]$), and output it as $\sigma$.
    If $m=1$, measure $\psi$ in the Hadamard basis to get the result $\{d_i\}_{i\in[n]}$ (where $d_i\in\bit^\ell$ for each $i\in[n]$), and output it as $\sigma$.
    \item 
    $\Ver_0(\pk,\sigma)\to\top/\bot:$
    Parse 
    $\pk=\{f(x_i^0),f(x_i^1)\}_{i\in[n]}$ and $\sigma=\{z_i\}_{i\in[n]}$. 
    If $f(z_i)\in\{f(x_i^0),f(x_i^1)\}$ for all $i\in[n]$, output $\top$.
    Otherwise, output $\bot$.
    \item 
    $\Ver_1(\sk,\sigma)\to\top/\bot:$
   Parse $\sk=\{c_i,x_i^0,x_i^1\}_{i\in[n]}$ and $\sigma=\{d_i\}_{i\in[n]}$.
    If $d_i\cdot(x_i^0\oplus x_i^1)=c_i$ for all $i\in[n]$, output $\top$. 
    Otherwise, output $\bot$.
\end{itemize}
The correctness is clear.
The security is also clear from \cref{thm:adaptive_hardcore_bit_amp}.
\end{proof}

\subsubsection{Two-tier quantum money}
Two-tier quantum money can be constructed from two-tier tokenized signature in a black-box way.
\begin{theorem}
If two-tier tokenized signatures exist, then two-tier quantum money exist.    
\end{theorem}

\begin{proof}
Let $(\KeyGen',\StateGen',\Sign,\Ver_0,\Ver_1)$    
be a two-tier tokenized signature. From it, we construct two-tier quantum money $(\KeyGen,\StateGen,\SemiVer,\FullVer)$ as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to(\sk,\pk):$
    Run $\KeyGen'(1^\secp)\to(\sk',\pk')$.
    Output $\sk\coloneqq \sk'$ and $\pk\coloneqq \pk'$.
    \item 
    $\StateGen(\sk)\to\psi:$
    Run $\StateGen'(\sk)\to\psi'$.
    Output $\psi\coloneqq\psi'$.
    \item 
    $\SemiVer(\pk,\psi)\to\top/\bot:$
    Run $\Sign(\psi,0)\to\sigma_0$.
    Run $\Ver_0(\pk,\sigma_0)$ and output its output.
     \item 
    $\FullVer(\sk,\psi)\to\top/\bot:$
    Run $\Sign(\psi,1)\to\sigma_1$.
    Run $\Ver_1(\sk,\sigma_1)$ and output its output.
\end{itemize}
Both correctness and security are clear.
\end{proof}

\if0
\begin{proof}
Let $f$ be a OWF. We construct two-tier quantum money as follows.
\begin{itemize}
     \item 
    $\KeyGen(1^\secp)\to (\sk,\pk):$
    Choose $x_i^0,x_i^1\gets\bit^\ell$ for each $i\in[n]$.
    Choose $c_i\gets\bit$ for each $i\in[n]$.
    Output $\sk\coloneqq\{c_i,x_i^0,x_i^1\}_{i\in[n]}$
    and $\pk\coloneqq\{f(x_i^0),f(x_i^1)\}_{i\in[n]}$.
    \item 
    $\StateGen(\sk)\to\psi:$
    Parse $\sk=\{c_i,x_i^0,x_i^1\}_{i\in[n]}$.
    Output $\psi\coloneqq\bigotimes_{i\in[n]}\frac{\ket{x_i^0}+(-1)^{c_i}\ket{x_i^1}}{\sqrt{2}}$. 
    \item 
    $\SemiVer(\pk,\psi)\to\top/\bot:$
    Parse 
    $\pk=\{f(x_i^0),f(x_i^1)\}_{i\in[n]}$. Measure all qubits of $\psi$ in the computational basis to get the result $\{z_i\}_{i\in[n]}$.
    If $z_i\in\{f(x_i^0),f(x_i^1)\}$ for all $i\in[n]$, output $\top$.
    Otherwise, output $\bot$.
    \item 
    $\FullVer(\sk,\psi)\to\top/\bot:$
   Parse $\sk=\{c_i,x_i^0,x_i^1\}_{i\in[n]}$.
    Measure all qubits of $\psi$ in the Hadamard basis to get the result $\{d_i\}_{i\in[n]}$.
    If $d_i\cdot(x_i^0\oplus x_i^1)=c_i$ for all $i\in[n]$, output $\top$. 
    Otherwise, output $\bot$.
\end{itemize}
The correctness is clear.
The security is shown from \cref{thm:adaptive_hardcore_bit_amp}.
\end{proof}
\fi



\subsubsection{Two-tier one-shot signatures}
Two-tier one-shot signatures can be constructed from subexponential LWE.
\begin{theorem}
Assuming the quantum subexponential hardness of the LWE problem, there exists two-tier one-shot signatures.  
\end{theorem}

\begin{proof}
To construct a two-tier one-shot signature scheme from LWE, we use NTCF families (see \Cref{def:NTCF}).

\paragraph{Construction.} 
\mor{Syntax has been changed, so the following proof should be modified.}
\alex{I changed it. Can you check if it's OK now?}
\mor{Thanks. The syntax will still change later, so it would be better not to finialize the proof here. Sorry for that! (I am currently struggling for
defining and constructing the revocable signing key one!}

Let $n = \omega(\log \lambda)$. Consider the following scheme.
\begin{itemize}

    \item $\Setup(1^\secp)$: Generate $(k_i,\mathsf{td}_i) \leftarrow \mathsf{NTCF}.\Gen_{\mathcal{F}}(1^\lambda)$ for $i \in [n]$ and set $(\pp,\sk):=(\{k_i\}_{i \in [n]}, \{ \mathsf{td}_i\}_{i \in [n]})$.
   
    \item 
    $\KeyGen(\pp)$:
    Parse $\pp = \{k_i\}_{i \in [n]}$. For each $i \in [n]$, generate a quantum state
$$
    \ket{\psi'_i} = \frac{1}{\sqrt{|\mathcal{X}|}} \sum_{x \in \mathcal{X}, y\in \mathcal{Y},
    b \in \bit}
\sqrt{(f'_{k_i,b}(x))(y)} \ket{b,x} \ket{y}
    $$
by using $\mathsf{Samp}_{\mathcal{F}}$, measure the last register to obtain $y_i \in \mathcal{Y}$, and let $\ket{\phi'_i}$ be the post-measurement state where the measured register is discarded. Output $(\vk,\sigk) = (\{y_i\}_{i \in [n]}, \{\ket{\phi'_i}\}_{i \in [n]})$.    
    \item 
    $\Sign(\sigk,m):$ on input $m \in \bit$, parse $\sigk$ as $ \{\ket{\phi'_i}\}_{i \in [n]}$ and then proceed as follows:
    \begin{itemize}
        \item if $m=0$: measure $\ket{\phi'_i}$ in the computational basis for $i \in [n]$, which results in measurement outcomes $\{(b_i,x_i)\}_{i \in [n]}$, and output $\sigma = \{(b_i,x_i)\}_{i \in [n]}$ as the signature.

         \item if $m=1$: measure $\ket{\phi'_i}$ in the Hadamard basis for $i \in [n]$, which results in measurement outcomes $\{(c_i,d_i)\}_{i \in [n]}$, and output $\sigma = \{(c_i,d_i)\}_{i \in [n]}$ as the signature.
    \end{itemize}
    
    \item 
    $\Ver_0(\pk,\vk,\sigma):$
    Parse $\pp = \{k_i\}_{i \in [n]}$, $\vk = \{y_i\}_{i \in [n]}$ and  $\sigma = \{(b_i,x_i)\}_{i \in [n]}$. Use the procedure $\mathsf{Chk}_{\mathcal{F}}$ in \Cref{def:NTCF} to determine if $y_i \in \mathsf{Supp}(f'_{k,b}(x_i))$ for all $i \in [n]$. Output $\top$ if it is the case, and output $\bot$ otherwise.
    \item 
    $\Ver_1(\pp,\sk,\sigma):$
    Parse $\pp = \{k_i\}_{i \in [n]}$, $\sk = \{ \mathsf{td}_i\}_{i \in [n]}$ and $\sigma = \{(c_i,d_i)\}_{i \in [n]}$. Then, compute $x_{i,\beta} \leftarrow \mathsf{Inv}_{\mathcal{F}}(\mathsf{td}_i, \beta, y_i)$ for every $i\in [n]$ and $\beta \in \bit$. Output $\top$, if $d_i \in \mathcal{G}_{k,0,x_{i,0}} \cap \mathcal{G}_{k,1,x_{i,1}}$ and $c_i = d_i \cdot (J(x_{i,0}) \oplus J(x_{i,1}))$ for all $i \in [n]$, and output $\bot$ otherwise.
\end{itemize}
The correctness of our two-tier one-shot signature scheme follows from the properties of the NTCF in \Cref{def:NTCF}. Security follows from the amplified adaptive hardcore bit property in \Cref{def:ampl-adaptive-hc}.
\end{proof}


\subsubsection{Two-tier quantum lightning}
It was shown in \cite{TCC:KitNisYam21} that two-tier quantum lightning can be constructed from the LWE assumption or the SIS assumption.
We show here that two-tier quantum lightning can be constructed from two-tier one-shot signatures in a black-box way:
\begin{theorem}
\label{thm:OSStoQL}
If two-tier one-shot signatures exist, then two-tier quantum lightning exist.    
\end{theorem}
\begin{proof}[Proof of \cref{thm:OSStoQL}]
Let $(\KeyGen',\StateGen',\Sign,\Ver_0,\Ver_1)$    
be a two-tier one-shot signature. From it, we construct two-tier quantum lightning $(\KeyGen,\StateGen,\SemiVer,\FullVer)$ as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to(\sk,\pk):$
    Run $\KeyGen'(1^\secp)\to(\sk',\pk')$.
    Output $\sk\coloneqq \sk'$ and $\pk\coloneqq \pk'$.
    \item 
    $\StateGen(\pk)\to\psi:$
    Run $\StateGen'(\pk)\to\psi'$.
    Output $\psi\coloneqq\psi'$.
    \item 
    $\SemiVer(\pk,\psi)\to\top/\bot:$
    Run $\Sign(\psi,0)\to\sigma_0$.
    Run $\Ver_0(\pk,\sigma_0)$ and output its output.
     \item 
    $\FullVer(\sk,\psi)\to\top/\bot:$
    Run $\Sign(\psi,1)\to\sigma_1$.
    Run $\Ver_1(\sk,\sigma_1)$ and output its output.
\end{itemize}
Both correctness and security are clear.
\end{proof}


We can also construct two-tier quantum lightning based on group actions~\cite{TCC:JQSY19}:
\begin{theorem}
\label{thm:GAtoQL}
Assuming group actions, two-tier quantum lightning exists.    
\end{theorem}
\mor{two-tier Quantum lightning's SemiVer accepts quantum state, but for signature, it should accept classical data.
So we should define a variant of two-tier quantum lightning where SemiVer accepts classical data.}
In order to show \cref{thm:GAtoQL}, we use {\it swap-trapdoor function pairs} (STF), which was introduced in \cite{EC:HhaMorYam23}.
STF can be constructed based on the group actions~\cite{TCC:JQSY19,EC:HhaMorYam23}.
The formal definition of STF is given as follows.
\begin{definition}[Swap-trapdoor function pair~\cite{EC:HhaMorYam23}]\label{def:STF}
A \emph{swap-trapdoor function pair (STF)} consists a set $(\setup,\eval,\swap)$ of algorithms such that
\begin{description}
\item[$\setup(1^\secp)\to(\pp,\td)$:] This is a PPT algorithm that takes the security parameter $1^\secp$ as input, and outputs a public parameter $\pp$ and a trapdoor $\td$. The public parameter $\pp$ specifies functions $f_b^{(\pp)}:\calX\rightarrow \calY$ for each $b\in\bit$. We often omit the dependence on $\pp$ and simply write $f_b$ when it is clear from the context.  
\item[$\eval(\pp,b,x)\to y$:] This is a deterministic classical polynomial-time algorithm that takes a public parameter $\pp$, a bit $b\in\bit$, and an element $x\in \calX$ as input, and outputs $y\in \calY$. 
\item[$\swap(\td,b,x)\to x'$:] This is a deterministic classical polynomial-time algorithm that takes a trapdoor $\td$, a bit $b\in \bit$, and an element $x\in \calX$ as input, and outputs $x'\in \calX$.
\end{description}
We require a STF to satisfy the following:

\smallskip\noindent\textbf{Evaluation correctness.}
For any $(\pp,\td)\gets \setup(1^\secp)$ , $b\in\bit$, and $x\in \calX$, we have $\eval(\pp,b,x)=f_b(x)$.

\smallskip\noindent\textbf{Swapping correctness.}
For any $(\pp,\td)\gets \setup(1^\secp)$, $b\in \bit$, and $x\in \calX$, 
 if we let $x'\gets \swap(\td,b,x)$, then we have $f_{b\oplus 1}(x')=f_b(x)$ and $\swap(\td,b\oplus 1,x')=x$.
In particular, $\swap(\td,b,\cdot)$ induces an efficiently computable and invertible one-to-one mapping between $f^{-1}_0(y)$ and $f^{-1}_1(y)$ for any $y\in \calY$. 
%\takashi{We may want to improve the explanation here to make the intuition clearer.}
 
%\smallskip\noindent\textbf{Claw-freeness.}
%For any non-uniform QPT algorithm $\A$, we have 
%\begin{align*}
%    \Pr[f_0(x_0)=f_1(x_1):(\pp,\td)\gets \setup(1^\secp),(x_0,x_1)\gets \A(\pp)]=\negl(\secp).
%\end{align*}

\smallskip\noindent\textbf{Efficient random sampling over $\calX$.} 
There is a PPT algorithm that samples an almost uniform element of $\calX$ (i.e., the distribution of the sample is statistically close to the uniform distribution). 

\smallskip\noindent\textbf{Efficient superposition over $\calX$.} 
There is a QPT algorithm
 that generates a state whose trace distance from $\ket{\calX}=\frac{1}{\sqrt{|\calX|}}\sum_{x\in\calX}|x\rangle$ is $\negl(\secp)$.

\smallskip\noindent\textbf{Claw-freeness.}
For any non-uniform QPT algorithm $\A$, 
\begin{align*}
    \Pr[f_0(x_0)=f_1(x_1):(\pp,\td)\gets \setup(1^\secp),(x_0,x_1)\gets \A(\pp)]=\negl(\secp).
\end{align*}

\smallskip\noindent\textbf{Conversion hardness.}
\mor{Maybe only claw-freeness is used?}
For any non-uniform QPT algorithm $\A$, 
\begin{align*}
    \Pr[f_1(x_1)=y:(\pp,\td)\gets \setup(1^\secp),x_0\gets \calX, y\seteq f_0(x_0),  x_1\gets \A(\pp,\ket{f_0^{-1}(y)})]=\negl(\secp)
\end{align*} 
where we remind that $\ket{f_0^{-1}(y)}\seteq\frac{1}{\sqrt{|f_0^{-1}(y)|}}\sum_{x\in f_0^{-1}(y)}\ket{x}$.  
 
 \end{definition}

\begin{remark}[A convention on ``Efficient random sampling over $\calX$'' and ``Efficient superposition over $\calX$'' properties]\label{rem:random_sampling_and_superposition}
In the rest of this paper, we assume that we can sample elements from \emph{exactly} the uniform distribution of $\calX$.  Similarly, we assume that we can \emph{exactly} generate $\ket{\calX}$ in QPT. They are just for simplifying the presentations of our results, and all the results hold with the above imperfect version with additive negligible loss for security or correctness. 
\end{remark}




\begin{proof}[Proof of \cref{thm:GAtoQL}]
Let $(\setup,\eval,\swap)$ be a SFT.
From it, we construct two-tier quantum lightning $(\KeyGen,\StateGen,\SemiVer,\FullVer)$ as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to(\sk,\pk):$
    Run $(\pp,\td)\gets\setup(1^\secp)$.
    Output $\pk\coloneqq\pp$ and $\sk\coloneqq(\pp,\td)$.
    \item 
    $\StateGen(\pk)\to(\psi,\snum):$
    Parse $\pk\coloneqq\pp$.
    For each $i\in[n]$, repeat the following:
    \begin{enumerate}
    \item
    Generate $\sum_{b\in\bit}\sum_{x\in\calX}\ket{b}\ket{x}\ket{\eval(\pp,b,x)}$.
    \item  
   Measure the third register in the computational basis
    to get the measurement result $y_i$.
    The post-measurement state is
    $\psi_i\coloneqq\ket{0}\otimes\sum_{x\in f_0^{-1}(y_i)}\ket{x}+\ket{1}\otimes\sum_{x\in f_1^{-1}(y_i)}\ket{x}$. 
    \end{enumerate}
    Output $\psi\coloneqq\bigotimes_{i\in[n]}\psi_i$ and $\snum\coloneqq\{y_i\}_{i\in[n]}$.
    \item 
    $\SemiVer(\pk,\psi,\snum)\to\top/\bot:$
    Parse $\pk\coloneqq\pp$, $\psi=\bigotimes_{i\in[n]}\psi_i$ and $\snum=\{y_i\}_{i\in[n]}$.
    Measure $\psi_i$ in the computational basis to get the result $(b_i,z_i)\in\bit\times\calX$ for each $i\in[n]$.
    If $\eval(\pp,b_i,z_i)=y_i$ for all $i\in[n]$, output $\top$. Otherwise, output $\bot$.
    \item 
    $\FullVer(\sk,\psi,\snum)\to\top/\bot:$
    Parse $\sk\coloneqq(\pp,\td)$, $\psi=\bigotimes_{i\in[n]}\psi_i$, and $\snum=\{y_i\}_{i\in[n]}$.
    For each $i\in[n]$, do the following:
    \begin{enumerate}
        \item 
    Apply unitary $U$ such that $U\ket{b}\ket{x}\ket{0...0}=\ket{b}\ket{x}\ket{\eval(\pp,b,x)}$ on $\psi_i\otimes\ket{0...0}\bra{0...0}$, and measure
    the third register in the computational basis.
    If the measurement result is not $y_i$,  output $\bot$ and abort.
   \item 
    Apply $\swap$ on the second register of the post-measurement state conditioned that the first register is 1.
    Measure the first register in the Hadamard basis. If the result is 1, output $\bot$ and abort.
    \end{enumerate}
    Output $\top$.
\end{itemize}
The correctness is clear. 
To show the security, we define the sequence of games, 
Hybrid 0 (\cref{hyb0}), 
Hybrid 1 (\cref{hyb1}), and
Hybrid 2 (\cref{hyb2}).
Hybrid 0 is the original security game.
For the sake of contradiction, we
assume that there exists a QPT adversary $\cA$ such that
\begin{align}
\label{assumption}
\Pr[{\rm Hybrid~0}\to\top]\ge\frac{1}{\poly(\secp)}.    
\end{align}

\protocol{Hybrid 0}
{Hybrid 0}
{hyb0}
{
\begin{enumerate}
    \item 
    The challenger $\cC$ runs $(\td,\pp)\gets\setup(1^\secp)$,
    and sends $\pp$ to $\cA$.
    \item 
    $\cA$ sends a quantum state $\psi_{\regF,\regS}$ over two registers $\regF$ and $\regS$ to $\cC$.
    The register $\regF$ consists of sub-registers $(\regF_1,...,\regF_n)$ and
    the register $\regS$ consists of sub-registers $(\regS_1,...,\regS_n)$.
    Each $\regF_i$ is a $(|\calX|+1)$-qubit register.
    Each $\regS_i$ is a $(|\calX|+1)$-qubit register.
    $\cA$ also sends $\{y_i\}_{i\in[n]}$ to $\cC$.
    \item 
    \label{SemiV}
    From $i=1$ to $n$, $\cC$ does the following:
    \begin{enumerate}
        \item 
    Measure the register $\regS_i$ in the computational basis to get the result $(b_i,z_i)\in\bit\times\calX$.
    \item
    If $\eval(\pp,b_i,z_i)\neq y_i$, output $\bot$ and abort.
    \end{enumerate}
\item 
\label{FullV}
    From $i=1$ to $n$, $\cC$ does the following: 
    \begin{enumerate}
    \item 
    Apply $U$ such that $U\ket{b}\ket{x}\ket{0...0}=\ket{b}\ket{x}\ket{\eval(\pp,b,x)}$ on $\regF_i\otimes\ket{0...0}\bra{0...0}$,
    and measure the ancilla register in the computational basis. If the result is not $y_i$, output $\bot$ and abort.
        \item 
    Apply $\swap$ on the second register of the post-measurement state conditioned that the first qubit is 1.
    Measure the first qubit in the Hadamard basis. If the result is 1, output $\bot$ and abort.
    \end{enumerate}
    \item
    Output $\top$.
\end{enumerate}
}



\protocol{Hybrid 1}
{Hybrid 1}
{hyb1}
{
\begin{enumerate}
    \item
    The same as Hybrid 0. 
    \item
    The same as Hybrid 0.
    \item 
    The same as Hybrid 0.
 \item 
    From $i=1$ to $n$, $\cC$ does the following: 
    \begin{enumerate}
    \item 
    Apply $U$ such that $U\ket{b}\ket{x}\ket{0...0}=\ket{b}\ket{x}\ket{\eval(\pp,b,x)}$ on $\regF_i\otimes\ket{0...0}\bra{0...0}$,
    and measure the ancilla register in the computational basis. If the result is not $y_i$, output $\bot$ and abort.
        \item 
    Apply $\swap$ on the second register of the post-measurement state conditioned that the first qubit is 1.
    Measure the state in the computational basis to get the result $(e_i,w_i)\in\bit\times\calX$.
    \end{enumerate}   
    \item
    If there is $i\in[n]$ such that $b_i\neq e_i$, output $\top$. Otherwise, output $\bot$.
\end{enumerate}
}

\protocol{Hybrid 2}
{Hybrid 2}
{hyb2}
{
\begin{enumerate}
    \item
    The same as Hybrid 1. 
    \item
    The same as Hybrid 1.
    \item 
    The same as Hybrid 1.
\item 
    From $i=1$ to $n$, $\cC$ does the following: 
    \begin{enumerate}
        \item 
    Apply $U$ such that $U\ket{b}\ket{x}\ket{0...0}=\ket{b}\ket{x}\ket{\eval(\pp,b,x)}$ on $\regF_i\otimes\ket{0...0}\bra{0...0}$,
    and measure the ancilla register in the computational basis. If the result is not $y_i$, output $\bot$ and abort.
        \item 
    Measure the register $\regF_i$ in the computational basis to get the result $(e_i,w_i)\in\bit\times\calX$.
    \end{enumerate}
    \item
    If there is $i\in[n]$ such that $b_i\neq e_i$, output $\top$. Otherwise, output $\bot$.
\end{enumerate}
}


\protocol{Hybrid 3}
{Hybrid 3}
{hyb3}
{
\begin{enumerate}
    \item
    The same as Hybrid 2. 
In addition, $\cC$ chooses $i^*\gets[n]$.
    \item
    The same as Hybrid 2.
    \item 
    The same as Hybrid 2.
    \item 
    The same as Hybrid 2.
\item 
    If $b_{i^*}\neq e_{i^*}$, output $\top$.
    Otherwise, output $\bot$.
\end{enumerate}
}




\begin{lemma}
\label{lem:01}
If 
$\Pr[{\rm Hybrid~0}\to\top]\ge\frac{1}{\poly(\secp)}$,
then
$\Pr[{\rm Hybrid~1}\to\top]\ge\frac{1}{\poly(\secp)}$.
\end{lemma}

\begin{proof}
We have
\begin{align}
  \epsilon&\coloneqq \Pr[\mbox{Hybrid 0}\to\top]\\
  &=\sum_{\pp,\td,b_1,...,b_n}\Pr[\pp,\td,b_1,...,b_n]
  \Tr[\Pi \rho_{b_1,...,b_n,\pp,\td}],
\end{align}
where $\Pr[\pp,\td,b_1,...,b_n]$ is the probability that
$(\pp,\td)$ is obtained, and
$\cC$ does not abort and $(b_1,...,b_n)$ is obtained in \cref{SemiV} of \cref{hyb0}.
$\rho_{b_1,...,b_n,\pp,\td}$ is the state of the register $\regF$ after the end of \cref{SemiV}.
$\Pi$ is the POVM element that $\cC$ does not abort in \cref{FullV} of \cref{hyb0}.
From the standard average argument, we have
\begin{align}
\sum_{(\pp,\td,b_1,...,b_n)\in G}\Pr[\pp,\td,b_1,...,b_n]
\ge\frac{\epsilon}{2},    
\label{average}
\end{align}
where
\begin{align}
G\coloneqq\Big\{(\pp,\td,b_1,...,b_n):
  \Tr\Big[\Pi\rho_{\pp,\td,b_1,...,b_n}\Big]\ge\frac{\epsilon}{2}
\Big\}.
\label{inG}
\end{align}
Define
\begin{align}
\Lambda_{b_1,...,b_n}    
\coloneqq
\sum_{(s_1,...,s_n)\in\bit^n\setminus (b_1,...,b_n)}
\bigotimes_{i=1}^n\ket{s_i}\bra{s_i}.
\end{align}
As is shown later, for any state $\rho$ and any $(b_1,...,b_n)\in\bit^n$, we have
 \begin{align}
 \label{PiLambda}
  \Tr[(\ket{+}\bra{+}^{\otimes n}\otimes I) \rho]
  \le
  2\Tr[(\Lambda_{b_1,...,b_n}\otimes I)\rho]+2^{-n+1}. 
\end{align}
Let $\rho'_{\pp,\td,b_1,...,b_n}$ be the state which is obtained by applying the controlled-$\swap$ on
$\rho_{\pp,\td,b_1,...,b_n}$.
Then
\begin{align}
&\Pr[\mbox{Hybrid 1}\to\top]\\
&=    
\sum_{\pp,\td,b_1,...,b_n}
\Pr[\pp,\td,b_1,...,b_n]
\Tr[(\Lambda_{b_1,...,b_n}\otimes I)\rho'_{\pp,\td,b_1,...,b_n}]\\
&\ge
\sum_{(\pp,\td,b_1,...,b_n)\in G}
\Pr[\pp,\td,b_1,...,b_n]
\Tr[(\Lambda_{b_1,...,b_n}\otimes I)\rho'_{\pp,\td,b_1,...,b_n}]\\
&\ge
\sum_{(\pp,\td,b_1,...,b_n)\in G}
\Pr[\pp,\td,b_1,...,b_n]
\Big(\frac{1}{2}\Tr\left[(\ket{+}\bra{+}^{\otimes n}\otimes I)\rho'_{\pp,\td,b_1,...,b_n}\right]
-2^{-n}\Big)\label{Pinisuru}\\
&\ge\frac{\epsilon}{2}\Big(\frac{\epsilon}{4}-2^{-n}\Big)\label{epsilon}\\
&\ge\frac{1}{\poly(\secp)}.
\end{align}
Here, to derive \cref{Pinisuru}, we have used \cref{PiLambda}.
To derive \cref{epsilon}, we have used \cref{average} and \cref{inG}.
\end{proof}

\begin{lemma}
\label{lem:12}
$\Pr[{\rm Hybrid~2}\to\top]=\Pr[{\rm Hybrid~1}\to\top]$.
\end{lemma}
\begin{proof}
The controlled $\swap$ operations do not change the distribution of $(e_1,...,e_n)$.
\end{proof}


\begin{lemma}
\label{lem:23}
$\Pr[{\rm Hybrid~3}\to\top]\ge\frac{1}{n}\Pr[{\rm Hybrid~2}\to\top]$.
\end{lemma}
\begin{proof}
It is trivial.
\end{proof}


In summary, from \cref{assumption} and \cref{lem:01,lem:12}, we conclude that
$\Pr[{\rm Hybrid~3}\to\top]\ge\frac{1}{\poly(\secp)}$.
From such $\cA$ of Hybrid 3, we construct a QPT adversary $\cB$ that breaks the claw-freeness of STF as in \cref{cB}.
It is easy to verify that
\begin{align}
\Pr[\cB~ \mbox{wins}]&\ge 
\Pr[{\rm Hybrid~3}\to\top]\\
&\ge\frac{1}{\poly(\secp)}.
\end{align}

\protocol{$\cB$}
{$\cB$}
{cB}
{
\begin{enumerate}
    \item 
    Get $\pp$ as input.
    \item 
    Run $(\regF,\regS,\{y_i\}_{i\in[n]})\gets\cA(\pp)$.
    Choose $i^*\gets[n]$.
    \item 
    Measure $\regS_{i^*}$ in the computational basis to get the result $(b_{i^*},z_{i^*})$.
    Measure $\regF_{i^*}$ in the computational basis to get the result $(e_{i^*},w_{i^*})$.
    \item 
    Output $(z_{i^*},w_{i^*})$.
\end{enumerate}
}





\end{proof}

\begin{proof}[Proof of \cref{PiLambda}]
\label{App:PiLambda}
Because of the linearity of $\Tr$, we have only to show it for pure states.
We have
\begin{align}
\Tr[(\ket{+}\bra{+}^{\otimes n}\otimes I) \ket{\psi}\bra{\psi}]
&=
\Big\|(\bra{+}^{\otimes n}\otimes I)\ket{\psi}\Big\|^2\\
&=
\frac{1}{2^n}\Big\|\sum_{s_1,...,s_n}(\bra{s_1,...,s_n}\otimes I)|\psi\rangle\Big\|^2\\
&=
\frac{1}{2^n}\Big\|\sum_{(s_1,...,s_n)\neq(b_1,...,b_n)}(\bra{s_1,...,s_n}\otimes I)|\psi\rangle
+(\bra{b_1,...,b_n}\otimes I)|\psi\rangle
\Big\|^2\\
&\le
\frac{1}{2^{n-1}}\Big\|\sum_{(s_1,...,s_n)\neq(b_1,...,b_n)}(\bra{s_1,...,s_n}\otimes I)|\psi\rangle\Big\|^2\\
&~~~~+\frac{1}{2^{n-1}}\Big\|(\bra{b_1,...,b_n}\otimes I)|\psi\rangle\Big\|^2\\
&\le
\frac{1}{2^{n-1}}(2^n-1)\sum_{(s_1,...,s_n)\neq (b_1,...,b_n)} \|(\bra{s_1,...,s_n}\otimes I)|\psi\rangle\|^2
+2^{-n+1}\\
&=
\frac{2^n-1}{2^{n-1}}\Tr[(\Lambda_{b_1,...,b_n}\otimes I)\ket{\psi}\bra{\psi}]
+2^{-n+1}\\
&\le
2\Tr[(\Lambda_{b_1,...,b_n}\otimes I)\ket{\psi}\bra{\psi}]
+2^{-n+1}.
\end{align}
Here, we have used the triangle inequality and Jensen's inequality.
\end{proof}


==> twotierquantumlightning_backup.tex <==
\section{Two-tier Quantum Lightning with Classical Semi-Verification from Group Actions}
Two-tier quantum lightning was introduced in \cite{TCC:KitNisYam21},
which is a variant of quantum lightning introduced in \cite{JC:Zhandry21}.
It was shown in \cite{TCC:KitNisYam21} that two-tier quantum lightning can be constructed from the LWE assumption or the SIS assumption.
%The main difference of quantum lightning from (publicly-verifiable) quantum money
%is that the security is guaranteed even if money states are generated by the adversary.
In this section, we give the definition of a variant of two-tier quantum lightning where semi-verification algorithm is classical, and
show that it can be constructed from group actions.
We also point out that it can be constructed from two-tier one-shot signatures in a black-box way.





\subsection{Group Actions}
Here we review basics of group actions~\cite{TCC:JQSY19}. 
First, group actions are defined as follows.
\begin{definition}[Group actions]
Let $G$ be a (not necessarily abelian) group, $S$ be a set, and $\star:G\times S \rightarrow S$ be a function where we write $g\star s$ to mean $\star(g,s)$. We say that $(G,S,\star)$ is a \emph{group action} if it satisfies the following:
\begin{enumerate}
    \item For the identity element $e\in G$ and any $s\in S$, we have $e\star s=s$.
    \item For any $g,h\in G$ and any $s\in S$, we have $(gh)\star s = g\star(h\star s)$.
\end{enumerate}
\end{definition}

\if0
We use the following notations. For $s\in S$, we denote by $G_s\subseteq G$ to mean the stabilizer subgroup with respect to $s$, i.e., 
\begin{align*}
    G_s\seteq \{g\in G: g\star s =s\}.
\end{align*}
For $g\in G$ and a subgroup $H\subseteq G$, we denote by $gH$ to mean the left coset with respect to $g$ and $H$, i.e., 
\begin{align*}
    gH\seteq \{gh\in G: h\in H\}.
\end{align*}
We denote by $\ket{G}$ to mean the uniform superposition over $G$, i.e.,
\begin{align*}
    \ket{G}\seteq \frac{1}{|G|^{1/2}}\sum_{g\in G}\ket{g}.
\end{align*}
Similarly, for $g\in G$ and a subgroup $H\subseteq G$, we denote by $\ket{gH}$ to mean the uniform superposition over $gH$, i.e.,
\begin{align*}
    \ket{gH}\seteq \frac{1}{|H|^{1/2}}\sum_{h\in H}\ket{gh}.
\end{align*}
\fi

To be useful for cryptography, we have to at least assume that basic operations about $(G,S,\star)$ have efficient algorithms. We require the following efficient algorithms similarly to \cite{TCC:JQSY19}.
\begin{definition}[Group actions with efficient algorithms]\label{def:GA_efficient}
%Let $\{(G_\secp ,S_\secp ,\star_\secp)\}_{\secp \in \mathbb{N}}$ be a family of group actions. 
%where we omit the dependence of the security parameter $\secp$ from the notation for simplicity. 
We say that a group action $(G,S,\star)$ has \emph{efficient algorithms} if it satisfies the following:\footnote{Strictly speaking, we have to consider a family $\{(G_\secp ,S_\secp ,\star_\secp)\}_{\secp \in \mathbb{N}}$ of group actions parameterized by the security parameter to meaningfully define the efficiency requirements. We omit the dependence on $\secp$ for notational simplicity throughout the paper.} 
\begin{itemize}
    \item[{\bf Unique representations:}] Each element of $G$ and $S$ can be represented as a bit string of length $\poly(\secp)$ in a unique manner. Thus, we identify these elements and their representations.
    \item[{\bf Group operations:}] There are classical deterministic polynomial-time algorithms that compute $gh$ from $g\in G$ and $h \in G$ and $g^{-1}$ from $g \in G$.
    \item[{\bf Group action:}] There is a classical deterministic polynomial-time algorithm that computes $g\star s$ from $g\in G$ and $s\in S$.
    \item[{\bf Efficient recognizability:}] There are classical deterministic polynomial-time algorithms that decide if a given bit string represents an element of $G$ or $S$, respectively.
    \item[{\bf Random sampling:}] There are PPT algorithms that sample almost uniform elements of $G$ or $S$ (i.e., the distribution of the sample is statistically close to the uniform distribution), respectively.
    \item[{\bf Superposition over $G$:}] There is a QPT algorithm that generates a state whose trace distance from $\ket{G}$ is $\negl(\secp)$. 
\end{itemize}
\end{definition}
\begin{remark}[A convention on ``Random sampling'' and ``Superposition over $G$'' properties]
In the rest of this paper, we assume that we can sample elements from \emph{exactly} uniform distributions of $G$ and $S$. Similarly, we assume that we can \emph{exactly} generate $\ket{G}$ in QPT. They are just for simplifying the presentations of our results, and all the results hold with the above imperfect version with additive negligible loss for security or correctness. 
\end{remark}

\begin{remark}
The above requirements are identical to those in \cite{TCC:JQSY19} except for the ``superposition over $G$'' property. 
We remark that all candidate constructions proposed in  \cite{TCC:JQSY19} satisfy this property. 
%Such group actions are formalized as effective group actions in \cite{AC:ADMP20}.
%Here, we augment their definition by an additional requirement that we can  
%Our formalization is based on that in \cite{AC:ADMP20}, but we remark that we also consider actions by non-abelian groups unlike them.
\end{remark}

We define one-wayness and pseudorandomness~\cite{TCC:JQSY19} as follows.
\begin{definition}[One-wayness]\label{def:one-way}
We say that a group action $(G,S,\star)$ with efficient algorithms is \emph{one-way} if for any non-uniform QPT adversary $\A$, we have 
\begin{align*}
    \Pr\left[
    g'\star s = g\star s
    :
    \begin{array}{l}
     s\gets S,
    g\gets G,
    g' \leftarrow \A(s,g\star s)
    \end{array}
    \right]=\negl(\secp).
\end{align*}
\end{definition}

\begin{definition}[Pseudorandomness]\label{def:PR}
We say that a group action $(G,S,\star)$ with efficient algorithms is \emph{pseudorandom} if it satisfies the following:
\begin{enumerate}
\item \label{item:orbit}
We have 
\begin{align*}
\Pr[\exists g\in G\text{~s.t.~}g\star s =t:s,t\gets S]=\negl(\secp).
\end{align*}
\item \label{item:PR}
For any non-uniform QPT adversary $\A$, we have 
\begin{align*}
    \left|
    \Pr\left[
    1\gets \A(s,t):
     s\gets S,
    g\gets G,
    t\seteq g\star s
    \right]
    -
    \Pr\left[
    1\gets \A(s,t):
     s,t\gets S
    \right]
    \right|
    =
    \negl(\secp).
\end{align*}
\end{enumerate}
\end{definition}
\begin{remark}[On \Cref{item:orbit}]
We require \Cref{item:orbit} to make \Cref{item:PR} non-trivial. For example, if $(G,S,\star)$ is transitive, i.e., for any $s,t\in S$, there is $g\in G$ such that $g\star s =t$, \Cref{item:PR} trivially holds because the distributions of $t=g\star s$ is uniformly distributed over $S$ for any fixed $s$ and random $g\gets G$.  
\end{remark}
\begin{remark}[Pseudorandom $\rightarrow$ One-way]
We remark that the pseudorandomness immediately implies the one-wayness as noted in \cite{TCC:JQSY19}. 
\end{remark}

\if0
\noindent\textbf{Instantiations.}
Ji et al. \cite{TCC:JQSY19} gave several candidate constructions of one-way and pseudorandom group actions with efficient algorithms based on general linear group actions on tensors. 
We briefly describe one of their candidates below. 
Let $\mathbb{F}$ be a finite field, and $k$, $d_1,d_2...,d_k$ be positive integers (which are typically set as 
$k=3$ and $d_1=d_2=d_3$). 
We set $G\seteq \prod_{j=1}^{k}GL_{d_j}(\mathbb{F})$, $S\seteq \bigotimes_{j=1}^{k} \mathbb{F}^{d_j}$, and define the group action by the matrix-vector multiplication as
\begin{align*}
    (M_j)_{j\in[k]} \star T\seteq \left(\bigotimes_{j=1}^{k}M_j\right) T
\end{align*}
for $(M_j)_{j\in[k]}\in \prod_{j=1}^{k}GL_{d_j}(\mathbb{F})$ and $T\in \bigotimes_{j=1}^{k} \mathbb{F}^{d_j}$. 
%Specifically,... \takashi{to be written} 
See \cite{TCC:JQSY19} for attempts of cryptanalysis and justification of the one-wayness and pseudorandomness. 
We remark that we introduced an additional requirement of the ``superposition over $G$'' property in \Cref{def:GA_efficient}, but their candidates satisfy this property. 
In their candidates, the group $G$ is a direct product of general linear groups over finite fields (or symmetric groups for one of the candidates), and a uniformly random matrix over finite fields is invertible with overwhelming probability for appropriate parameters. 
\fi

\if0
Alamati et al. \cite{AC:ADMP20} introduced a similar formalization of cryptographic group actions as an abstraction of isogeny-based cryptography. However, there are several differences between our and their requirements. Notably, they do not require unique representation for elements of $G$ and efficient computability of the action by any group element. This is because the isogeny-based group action is not known to satisfy them. Thus, we cannot capture isogeny-based group action by our definition. We might be able to capture it by relaxing the requirements for group actions similarly to \cite{AC:ADMP20}.
However, we do not do so because our motivation here is to construct (quantum) PKE schemes, whose isogeny-based construction are already known even without relying on quantum ciphertexts~\cite{Couveignes06,PQCRYPTO:JaoDeFo11,AC:CLMPR18}. 

% which can be constructed even without relying on quantum ciphertexts based on isogeny~\cite{Couveignes06,PQCRYPTO:JaoDeFo11,AC:CLMPR18}. 


%However, a problem is that graph isomorphism problem is easy for a uniformly random instance \takashi{citation}, and thus group actions based on it cannot satisfy the one-wayness where $s\gets S$ is uniformly chosen for the instance generation. On the other hand, the one-wayness with a fixed $s$ may hold since there is no known QPT algorithm that solves graph isomorphism problem in the worst case. We note that such a variant of one-wayness suffices for our applications. However, since there is a (classical) quasi-polynomial time algorithm that solves graph ismorphism in the worst case~\cite{STOC:Babai16}, one-wayness of group actions based on it can be broken in quasi-polynomial time. Though this is not an attack in the standard sense in cryptography where the adversary is required to be (probabilistic) polynomial-time, quasi-polynomial time attacks are also often considered to be fatal. For this reason, we do not consider the instantiation based on graph ismorphism and simply consider uniform $s\in S$ in the definition of one-wayness.\footnote{A similar remark can be found in \cite[Remark~1]{TCC:JQSY19}}. 

Brassard and Yung~\cite{C:BraYun90} proposed cryptographic group actions based on the hardness of graph isomorphism,
discrete logarithm, or factoring. However, it turns out that the graph isomorphism problem can be solved in (classical) quasi polynomial-time~\cite{STOC:Babai16}\footnote{Another issue is that the graph isomorphism problem is easy for a uniformly random instance, and thus it cannot satisfy the one-wayness as defined in \Cref{def:one-way}. If we modify the definition of the one-wayness so that we choose the hardest instance $s\in S$, the graph isomorphism-based construction may satisfy it, and such a version suffices for our applications. However, since such a construction can be broken in quasi-polynomial time by Babai's algorithm \cite{STOC:Babai16}, we do not consider the instantiation based on graph ismorphism and simply consider uniform $s\in S$ in the definition of one-wayness. A similar remark can be found in \cite[Remark~1]{TCC:JQSY19}.} and discrete logarithm and factoring problems can be solved in QPT~\cite{Shor99}.
\fi

%A construction of cryptographic group actions based on the hardness of the graph isomorphism problem is proposed in \cite{C:BraYun90}. However, a (classical) quasi polynomial-time algorithm to solve the graph isomorphism problem was found~\cite{STOC:Babai16}.\footnote{Another issue is that the graph isomorphism problem is easy for a uniformly random instance, and thus it cannot satisfy the one-wayness as defined in \Cref{def:one-way}. We modify the definition of the one-wayness so that we choose the hardest instance $s\in S$, the graph isomorphism-based construction may satisfy it, and such a version suffices for our applications. However, since such a construction can be broken in quasi-polynomial time by Babai's algorithm \cite{STOC:Babai16}, we do not consider the instantiation based on graph ismorphism and simply consider uniform $s\in S$ in the definition of one-wayness. We note that a similar remark can be found in \cite[Remark~1]{TCC:JQSY19}.}  


%Finally, we mention that cryptographic group actions based on the hardness of discrete logarithm or factoring were given in \cite{C:BraYun90}. However, since these problem can be solved in quantunm polynomial-time by Shor's algorithm \cite{Shor99}, they are not suitable for our applications. 



\subsection{Swap-Trapdoor Functions Pairs}
In order to show the construction of two-tier quantum lightning with classical semi-verification from group actions, it is convenient to
use {\it swap-trapdoor function pairs} (STF), which was introduced in \cite{EC:HhaMorYam23}.
STF can be constructed based on the group actions~\cite{TCC:JQSY19,EC:HhaMorYam23}.
The formal definition of STF is given as follows.
\begin{definition}[Swap-trapdoor function pair~\cite{EC:HhaMorYam23}]\label{def:STF}
A \emph{swap-trapdoor function pair (STF)} consists a set $(\setup,\eval,\swap)$ of algorithms such that
\begin{description}
\item[$\setup(1^\secp)\to(\pp,\td)$:] This is a PPT algorithm that takes the security parameter $1^\secp$ as input, and outputs a public parameter $\pp$ and a trapdoor $\td$. The public parameter $\pp$ specifies functions $f_b^{(\pp)}:\calX\rightarrow \calY$ for each $b\in\bit$. We often omit the dependence on $\pp$ and simply write $f_b$ when it is clear from the context.  
\item[$\eval(\pp,b,x)\to y$:] This is a deterministic classical polynomial-time algorithm that takes a public parameter $\pp$, a bit $b\in\bit$, and an element $x\in \calX$ as input, and outputs $y\in \calY$. 
\item[$\swap(\td,b,x)\to x'$:] This is a deterministic classical polynomial-time algorithm that takes a trapdoor $\td$, a bit $b\in \bit$, and an element $x\in \calX$ as input, and outputs $x'\in \calX$.
\end{description}
We require a STF to satisfy the following:

\smallskip\noindent\textbf{Evaluation correctness.}
For any $(\pp,\td)\gets \setup(1^\secp)$ , $b\in\bit$, and $x\in \calX$, we have $\eval(\pp,b,x)=f_b(x)$.

\smallskip\noindent\textbf{Swapping correctness.}
For any $(\pp,\td)\gets \setup(1^\secp)$, $b\in \bit$, and $x\in \calX$, 
 if we let $x'\gets \swap(\td,b,x)$, then we have $f_{b\oplus 1}(x')=f_b(x)$ and $\swap(\td,b\oplus 1,x')=x$.
In particular, $\swap(\td,b,\cdot)$ induces an efficiently computable and invertible one-to-one mapping between $f^{-1}_0(y)$ and $f^{-1}_1(y)$ for any $y\in \calY$. 
%\takashi{We may want to improve the explanation here to make the intuition clearer.}
 
%\smallskip\noindent\textbf{Claw-freeness.}
%For any non-uniform QPT algorithm $\A$, we have 
%\begin{align*}
%    \Pr[f_0(x_0)=f_1(x_1):(\pp,\td)\gets \setup(1^\secp),(x_0,x_1)\gets \A(\pp)]=\negl(\secp).
%\end{align*}

\smallskip\noindent\textbf{Efficient random sampling over $\calX$.} 
There is a PPT algorithm that samples an almost uniform element of $\calX$ (i.e., the distribution of the sample is statistically close to the uniform distribution). 

\smallskip\noindent\textbf{Efficient superposition over $\calX$.} 
There is a QPT algorithm
 that generates a state whose trace distance from $\ket{\calX}=\frac{1}{\sqrt{|\calX|}}\sum_{x\in\calX}|x\rangle$ is $\negl(\secp)$.

\smallskip\noindent\textbf{Claw-freeness.}
For any non-uniform QPT algorithm $\A$, 
\begin{align*}
    \Pr[f_0(x_0)=f_1(x_1):(\pp,\td)\gets \setup(1^\secp),(x_0,x_1)\gets \A(\pp)]=\negl(\secp).
\end{align*}

\smallskip\noindent\textbf{Conversion hardness.}
\mor{Maybe only claw-freeness is used?}\takashi{I believe so.}
For any non-uniform QPT algorithm $\A$, 
\begin{align*}
    \Pr[f_1(x_1)=y:(\pp,\td)\gets \setup(1^\secp),x_0\gets \calX, y\seteq f_0(x_0),  x_1\gets \A(\pp,\ket{f_0^{-1}(y)})]=\negl(\secp)
\end{align*} 
where we remind that $\ket{f_0^{-1}(y)}\seteq\frac{1}{\sqrt{|f_0^{-1}(y)|}}\sum_{x\in f_0^{-1}(y)}\ket{x}$.  
 
 \end{definition}

\begin{remark}[A convention on ``Efficient random sampling over $\calX$'' and ``Efficient superposition over $\calX$'' properties]\label{rem:random_sampling_and_superposition}
In the rest of this paper, we assume that we can sample elements from \emph{exactly} the uniform distribution of $\calX$.  Similarly, we assume that we can \emph{exactly} generate $\ket{\calX}$ in QPT. They are just for simplifying the presentations of our results, and all the results hold with the above imperfect version with additive negligible loss for security or correctness. 
\end{remark}



A STF can be constructed from group actions. Let $(G,S,\star)$ be a group action with efficient algorithms (as defined in \Cref{def:GA_efficient}). Then, we construct a STF as follows.

\begin{description}
\item[$\setup(1^\secp)$:] Generate $s_0\gets S$ and $g\gets G$, set $s_1\seteq g\star s_0$, and output $\pp\seteq (s_0,s_1)$ and $\td\seteq g$. 
For $b\in \bit$, we define $f_b:G\rightarrow S$ by 
    $f_b(h)\seteq h\star s_b$.
\item[$\eval(\pp=(s_0,s_1),b,h)$:] Output $f_b(h)=h\star s_b$. 
\item[$\swap(\td=g,b,h)$:] 
If $b=0$, output $hg^{-1}$. If $b=1$, output $hg$. 
\end{description}

\if0
The evaluation correctness is trivial. The swapping correctness can be seen as follows: For any $h\in G$, $f_1(\swap(\td,0,h))=f_1(hg^{-1})=(hg^{-1})\star s_1 = h \star s_0 = f_0(h)$. Similarly, for any $h\in G$,  $f_0(\swap(\td,1,h))=f_0(hg)=(hg)\star s_0 = h \star s_1 = f_1(h)$. For any $h\in G$, $\swap(\td,1,\swap(\td,0,h))=\swap(\td,1,hg^{-1})=(hg^{-1})g=h$. 
The efficient sampling and efficient superposition properties directly follow from the corresponding properties of the group action.
\fi

In \cite{EC:HhaMorYam23}, the following theorem is shown.
\begin{theorem}[\cite{EC:HhaMorYam23}]\label{thm:GA_to_STF}
The following hold:
\begin{enumerate}
    \item If $(G,S,\star)$ is one-way, then $(\setup,\eval,\swap)$ is claw-free. \label{item:OW_to_CF}
    \item If $(G,S,\star)$ is pseudorandom, then $(\setup,\eval,\swap)$ is conversion hard. \label{item:PR_to_CH}\mor{may be conversion hardness will not be used}
\end{enumerate}
\end{theorem}


\subsection{Definition of two-tier quantum lightning with classical semi-verification}
The formal definition of two-tier quantum lightning with classical semi-verification is given as follows.
The difference from the original two-tier quantum lightning \cite{TCC:KitNisYam21} is that the semi-verification algorithm $\SemiVer$ accepts a classical certificate $\cert$
instead of a quantum state $\psi$, and there is an additional QPT algorithm $\Del$ that outputs $\cert$ on input $\psi$.
\begin{definition}[Two-tier quantum lightning with classical semi-verification]
Two-tier quantum lighting with classical semi-verification is a set $(\KeyGen,\StateGen,\Del,\SemiVer,\FullVer)$
of algorithms such that
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to(\sk,\pk):$
    It is a QPT algorithm that, on input the security parameter $\secp$, outputs
    a classical secret key $\sk$ and a classical public key $\pk$.
    \item 
    $\StateGen(\pk)\to(\psi,\snum):$
    It is a QPT algorithm that, on input $\pk$, outputs 
    a quantum state $\psi$ and a classical serial number $\snum$.
    \item 
    $\Del(\psi)\to\cert:$
    It is a QPT algorithm that, on input $\psi$, outputs a classical certificate $\cert$.
    \item 
    $\SemiVer(\pk,\cert,\snum)\to\top/\bot:$
    It is a QPT algorithm that, on input $\pk$, $\cert$, and $\snum$, outputs $\top/\bot$.
    \item 
    $\FullVer(\sk,\psi,\snum)\to\top/\bot:$
    It is a QPT algorithm that, on input $\sk$, $\psi$, and $\snum$, outputs $\top/\bot$.
\end{itemize}
We require the following properties.

\paragraph{Correctness:}
\begin{align}
\Pr\left[\top\gets\SemiVer(\pk,\cert,\snum):
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
(\psi,\snum)\gets\StateGen(\pk)\\
\cert\gets\Del(\psi)
\end{array}
\right]\ge1-\negl(\secp)    
\end{align}
and
\begin{align}
\Pr\left[\top\gets\FullVer(\sk,\psi,\snum):
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
(\psi,\snum)\gets\StateGen(\pk)\\
\end{array}
\right]\ge1-\negl(\secp).
\end{align}

\paragraph{Security:}
For any QPT adversary $\cA$,
\begin{align}
\Pr\left[
\top\gets\SemiVer(\pk,\cert,\snum)
\wedge
\top\gets\FullVer(\sk,\psi,\snum)
:
\begin{array}{rr}
(\sk,\pk)\gets\KeyGen(1^\secp)\\
(\cert,\psi,\snum)\gets\cA(\pk)\\
\end{array}
\right]\le\negl(\secp).    
\end{align}
\end{definition}

\if0
\begin{remark}
In the definition in \cite{TCC:KitNisYam21}, $\SemiVer$ also outputs a quantum state $\psi'$,
but in this paper, we consider a simpler syntax where
$\SemiVer$ outputs only $\top/\bot$.
\end{remark}
\fi




\subsection{Construction from group actions}
Here we construct two-tier quantum lightning with classical semi-verification from STF (and therefore from group actions).
\begin{theorem}
\label{thm:GAtoQL}
Assuming group actions \mor{that satisfy the one-wayness}, two-tier quantum lightning with classical semi-verification exists.    
\end{theorem}



\begin{proof}[Proof of \cref{thm:GAtoQL}]
Let $(\setup,\eval,\swap)$ be a SFT \mor{that satisfies the claw-free property. Such SFT exists if
group actions that satisfy one-wayness exist.}
From it, we construct two-tier quantum lightning with classical semi-verification $(\KeyGen,\StateGen,\Del,\SemiVer,\FullVer)$ as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to(\sk,\pk):$
    Run $(\pp,\td)\gets\setup(1^\secp)$.
    Output $\pk\coloneqq\pp$ and $\sk\coloneqq(\pp,\td)$.
    \item 
    $\StateGen(\pk)\to(\psi,\snum):$
    Parse $\pk\coloneqq\pp$.
    For each $i\in[n]$, repeat the following:
    \begin{enumerate}
    \item
    Generate $\sum_{b\in\bit}\sum_{x\in\calX}\ket{b}\ket{x}\ket{\eval(\pp,b,x)}$.
    \item  
   Measure the third register in the computational basis
    to get the measurement result $y_i$.
    The post-measurement state is
    $\psi_i\coloneqq\ket{0}\otimes\sum_{x\in f_0^{-1}(y_i)}\ket{x}+\ket{1}\otimes\sum_{x\in f_1^{-1}(y_i)}\ket{x}$. 
    \end{enumerate}
    Output $\psi\coloneqq\bigotimes_{i\in[n]}\psi_i$ and $\snum\coloneqq\{y_i\}_{i\in[n]}$.
     \item 
    $\Del(\psi)\to\cert:$
    Parse $\psi=\bigotimes_{i\in[n]}\psi_i$.
    Measure $\psi_i$ in the computational basis to get the result $(b_i,z_i)\in\bit\times\calX$ for each $i\in[n]$.
    Output $\cert\coloneqq \{b_i,z_i\}_{i\in[n]}$.
    \item 
    $\SemiVer(\pk,\cert,\snum)\to\top/\bot:$
    Parse $\pk\coloneqq\pp$, $\cert=\{b_i,z_i\}_{i\in[n]}$ and $\snum=\{y_i\}_{i\in[n]}$.
    If $\eval(\pp,b_i,z_i)=y_i$ for all $i\in[n]$, output $\top$. Otherwise, output $\bot$.
    
    \item 
    $\FullVer(\sk,\psi,\snum)\to\top/\bot:$
    Parse $\sk\coloneqq(\pp,\td)$, $\psi=\bigotimes_{i\in[n]}\psi_i$, and $\snum=\{y_i\}_{i\in[n]}$.
    For each $i\in[n]$, do the following:
    \begin{enumerate}
        \item 
    Apply unitary $U$ such that $U\ket{b}\ket{x}\ket{0...0}=\ket{b}\ket{x}\ket{\eval(\pp,b,x)}$ on $\psi_i\otimes\ket{0...0}\bra{0...0}$, and measure
    the third register in the computational basis.
    If the measurement result is not $y_i$,  output $\bot$ and abort.
   \item 
    Apply $\swap$ on the second register of the post-measurement state conditioned that the first register is 1.
    Measure the first register in the Hadamard basis. If the result is 1, output $\bot$ and abort.
    \end{enumerate}
    Output $\top$.
\end{itemize}
The correctness is clear. 
To show the security, we define the sequence of games, 
Hybrid 0 (\cref{hyb0}), 
Hybrid 1 (\cref{hyb1}), and
Hybrid 2 (\cref{hyb2}).
Hybrid 0 is the original security game.
For the sake of contradiction, we
assume that there exists a QPT adversary $\cA$ such that
\begin{align}
\label{assumption}
\Pr[{\rm Hybrid~0}\to\top]\ge\frac{1}{\poly(\secp)}.    
\end{align}

\protocol{Hybrid 0}
{Hybrid 0}
{hyb0}
{
\begin{enumerate}
    \item 
    The challenger $\cC$ runs $(\td,\pp)\gets\setup(1^\secp)$,
    and sends $\pp$ to $\cA$.
    \item 
    $\cA$ sends a quantum state $\psi_{\regF,\regS}$ over two registers $\regF$ and $\regS$ to $\cC$.
    The register $\regF$ consists of sub-registers $(\regF_1,...,\regF_n)$ and
    the register $\regS$ consists of sub-registers $(\regS_1,...,\regS_n)$.
    Each $\regF_i$ is a $(|\calX|+1)$-qubit register.
    Each $\regS_i$ is a $(|\calX|+1)$-qubit register.
    $\cA$ also sends $\{y_i\}_{i\in[n]}$ to $\cC$.
    \item 
    \label{SemiV}
    From $i=1$ to $n$, $\cC$ does the following:
    \begin{enumerate}
        \item 
    Measure the register $\regS_i$ in the computational basis to get the result $(b_i,z_i)\in\bit\times\calX$.
    \item
    If $\eval(\pp,b_i,z_i)\neq y_i$, output $\bot$ and abort.
    \end{enumerate}
\item 
\label{FullV}
    From $i=1$ to $n$, $\cC$ does the following: 
    \begin{enumerate}
    \item 
    Apply $U$ such that $U\ket{b}\ket{x}\ket{0...0}=\ket{b}\ket{x}\ket{\eval(\pp,b,x)}$ on $\regF_i\otimes\ket{0...0}\bra{0...0}$,
    and measure the ancilla register in the computational basis. If the result is not $y_i$, output $\bot$ and abort.
        \item 
    Apply $\swap$ on the second register of the post-measurement state conditioned that the first qubit is 1.
    Measure the first qubit in the Hadamard basis. If the result is 1, output $\bot$ and abort.
    \end{enumerate}
    \item
    Output $\top$.
\end{enumerate}
}



\protocol{Hybrid 1}
{Hybrid 1}
{hyb1}
{
\begin{enumerate}
    \item
    The same as Hybrid 0. 
    \item
    The same as Hybrid 0.
    \item 
    The same as Hybrid 0.
 \item 
    From $i=1$ to $n$, $\cC$ does the following: 
    \begin{enumerate}
    \item 
    Apply $U$ such that $U\ket{b}\ket{x}\ket{0...0}=\ket{b}\ket{x}\ket{\eval(\pp,b,x)}$ on $\regF_i\otimes\ket{0...0}\bra{0...0}$,
    and measure the ancilla register in the computational basis. If the result is not $y_i$, output $\bot$ and abort.
        \item 
    Apply $\swap$ on the second register of the post-measurement state conditioned that the first qubit is 1.
    Measure the state in the computational basis to get the result $(e_i,w_i)\in\bit\times\calX$.
    \end{enumerate}   
    \item
    If there is $i\in[n]$ such that $b_i\neq e_i$, output $\top$. Otherwise, output $\bot$.
\end{enumerate}
}

\protocol{Hybrid 2}
{Hybrid 2}
{hyb2}
{
\begin{enumerate}
    \item
    The same as Hybrid 1. 
    \item
    The same as Hybrid 1.
    \item 
    The same as Hybrid 1.
\item 
    From $i=1$ to $n$, $\cC$ does the following: 
    \begin{enumerate}
        \item 
    Apply $U$ such that $U\ket{b}\ket{x}\ket{0...0}=\ket{b}\ket{x}\ket{\eval(\pp,b,x)}$ on $\regF_i\otimes\ket{0...0}\bra{0...0}$,
    and measure the ancilla register in the computational basis. If the result is not $y_i$, output $\bot$ and abort.
        \item 
    Measure the register $\regF_i$ in the computational basis to get the result $(e_i,w_i)\in\bit\times\calX$.
    \end{enumerate}
    \item
    If there is $i\in[n]$ such that $b_i\neq e_i$, output $\top$. Otherwise, output $\bot$.
\end{enumerate}
}


\protocol{Hybrid 3}
{Hybrid 3}
{hyb3}
{
\begin{enumerate}
    \item
    The same as Hybrid 2. 
In addition, $\cC$ chooses $i^*\gets[n]$.
    \item
    The same as Hybrid 2.
    \item 
    The same as Hybrid 2.
    \item 
    The same as Hybrid 2.
\item 
    If $b_{i^*}\neq e_{i^*}$, output $\top$.
    Otherwise, output $\bot$.
\end{enumerate}
}




\begin{lemma}
\label{lem:01}
If 
$\Pr[{\rm Hybrid~0}\to\top]\ge\frac{1}{\poly(\secp)}$,
then
$\Pr[{\rm Hybrid~1}\to\top]\ge\frac{1}{\poly(\secp)}$.
\end{lemma}

\begin{proof}
We have
\begin{align}
  \epsilon&\coloneqq \Pr[\mbox{Hybrid 0}\to\top]\\
  &=\sum_{\pp,\td,b_1,...,b_n}\Pr[\pp,\td,b_1,...,b_n]
  \Tr[\Pi \rho_{b_1,...,b_n,\pp,\td}],
\end{align}
where $\Pr[\pp,\td,b_1,...,b_n]$ is the probability that
$(\pp,\td)$ is obtained, and
$\cC$ does not abort and $(b_1,...,b_n)$ is obtained in \cref{SemiV} of \cref{hyb0}.
$\rho_{b_1,...,b_n,\pp,\td}$ is the state of the register $\regF$ after the end of \cref{SemiV}.
$\Pi$ is the POVM element that $\cC$ does not abort in \cref{FullV} of \cref{hyb0}.
From the standard average argument, we have
\begin{align}
\sum_{(\pp,\td,b_1,...,b_n)\in G}\Pr[\pp,\td,b_1,...,b_n]
\ge\frac{\epsilon}{2},    
\label{average}
\end{align}
where
\begin{align}
G\coloneqq\Big\{(\pp,\td,b_1,...,b_n):
  \Tr\Big[\Pi\rho_{\pp,\td,b_1,...,b_n}\Big]\ge\frac{\epsilon}{2}
\Big\}.
\label{inG}
\end{align}
Define
\begin{align}
\Lambda_{b_1,...,b_n}    
\coloneqq
\sum_{(s_1,...,s_n)\in\bit^n\setminus (b_1,...,b_n)}
\bigotimes_{i=1}^n\ket{s_i}\bra{s_i}.
\end{align}
As is shown later, for any state $\rho$ and any $(b_1,...,b_n)\in\bit^n$, we have
 \begin{align}
 \label{PiLambda}
  \Tr[(\ket{+}\bra{+}^{\otimes n}\otimes I) \rho]
  \le
  2\Tr[(\Lambda_{b_1,...,b_n}\otimes I)\rho]+2^{-n+1}. 
\end{align}
Let $\rho'_{\pp,\td,b_1,...,b_n}$ be the state which is obtained by applying the controlled-$\swap$ on
$\rho_{\pp,\td,b_1,...,b_n}$.
Then
\begin{align}
&\Pr[\mbox{Hybrid 1}\to\top]\\
&=    
\sum_{\pp,\td,b_1,...,b_n}
\Pr[\pp,\td,b_1,...,b_n]
\Tr[(\Lambda_{b_1,...,b_n}\otimes I)\rho'_{\pp,\td,b_1,...,b_n}]\\
&\ge
\sum_{(\pp,\td,b_1,...,b_n)\in G}
\Pr[\pp,\td,b_1,...,b_n]
\Tr[(\Lambda_{b_1,...,b_n}\otimes I)\rho'_{\pp,\td,b_1,...,b_n}]\\
&\ge
\sum_{(\pp,\td,b_1,...,b_n)\in G}
\Pr[\pp,\td,b_1,...,b_n]
\Big(\frac{1}{2}\Tr\left[(\ket{+}\bra{+}^{\otimes n}\otimes I)\rho'_{\pp,\td,b_1,...,b_n}\right]
-2^{-n}\Big)\label{Pinisuru}\\
&\ge\frac{\epsilon}{2}\Big(\frac{\epsilon}{4}-2^{-n}\Big)\label{epsilon}\\
&\ge\frac{1}{\poly(\secp)}.
\end{align}
Here, to derive \cref{Pinisuru}, we have used \cref{PiLambda}.
To derive \cref{epsilon}, we have used \cref{average} and \cref{inG}.
\end{proof}

\begin{lemma}
\label{lem:12}
$\Pr[{\rm Hybrid~2}\to\top]=\Pr[{\rm Hybrid~1}\to\top]$.
\end{lemma}
\begin{proof}
The controlled $\swap$ operations do not change the distribution of $(e_1,...,e_n)$.
\end{proof}


\begin{lemma}
\label{lem:23}
$\Pr[{\rm Hybrid~3}\to\top]\ge\frac{1}{n}\Pr[{\rm Hybrid~2}\to\top]$.
\end{lemma}
\begin{proof}
It is trivial.
\end{proof}


In summary, from \cref{assumption} and \cref{lem:01,lem:12}, we conclude that
$\Pr[{\rm Hybrid~3}\to\top]\ge\frac{1}{\poly(\secp)}$.
From such $\cA$ of Hybrid 3, we construct a QPT adversary $\cB$ that breaks the claw-freeness of STF as in \cref{cB}.
It is easy to verify that
\begin{align}
\Pr[\cB~ \mbox{wins}]&\ge 
\Pr[{\rm Hybrid~3}\to\top]\\
&\ge\frac{1}{\poly(\secp)}.
\end{align}

\protocol{$\cB$}
{$\cB$}
{cB}
{
\begin{enumerate}
    \item 
    Get $\pp$ as input.
    \item 
    Run $(\regF,\regS,\{y_i\}_{i\in[n]})\gets\cA(\pp)$.
    Choose $i^*\gets[n]$.
    \item 
    Measure $\regS_{i^*}$ in the computational basis to get the result $(b_{i^*},z_{i^*})$.
    Measure $\regF_{i^*}$ in the computational basis to get the result $(e_{i^*},w_{i^*})$.
    \item 
    Output $(z_{i^*},w_{i^*})$.
\end{enumerate}
}





\end{proof}

\begin{proof}[Proof of \cref{PiLambda}]
\label{App:PiLambda}
Because of the linearity of $\Tr$, we have only to show it for pure states.
We have
\begin{align}
\Tr[(\ket{+}\bra{+}^{\otimes n}\otimes I) \ket{\psi}\bra{\psi}]
&=
\Big\|(\bra{+}^{\otimes n}\otimes I)\ket{\psi}\Big\|^2\\
&=
\frac{1}{2^n}\Big\|\sum_{s_1,...,s_n}(\bra{s_1,...,s_n}\otimes I)|\psi\rangle\Big\|^2\\
&=
\frac{1}{2^n}\Big\|\sum_{(s_1,...,s_n)\neq(b_1,...,b_n)}(\bra{s_1,...,s_n}\otimes I)|\psi\rangle
+(\bra{b_1,...,b_n}\otimes I)|\psi\rangle
\Big\|^2\\
&\le
\frac{1}{2^{n-1}}\Big\|\sum_{(s_1,...,s_n)\neq(b_1,...,b_n)}(\bra{s_1,...,s_n}\otimes I)|\psi\rangle\Big\|^2\\
&~~~~+\frac{1}{2^{n-1}}\Big\|(\bra{b_1,...,b_n}\otimes I)|\psi\rangle\Big\|^2\\
&\le
\frac{1}{2^{n-1}}(2^n-1)\sum_{(s_1,...,s_n)\neq (b_1,...,b_n)} \|(\bra{s_1,...,s_n}\otimes I)|\psi\rangle\|^2
+2^{-n+1}\\
&=
\frac{2^n-1}{2^{n-1}}\Tr[(\Lambda_{b_1,...,b_n}\otimes I)\ket{\psi}\bra{\psi}]
+2^{-n+1}\\
&\le
2\Tr[(\Lambda_{b_1,...,b_n}\otimes I)\ket{\psi}\bra{\psi}]
+2^{-n+1}.
\end{align}
Here, we have used the triangle inequality and Jensen's inequality.
\end{proof}

\subsection{Constructions from two-tier one-shot signatures}
It was shown in \cite{TCC:KitNisYam21} that two-tier quantum lightning can be constructed from the LWE assumption or the SIS assumption.
We show here that two-tier quantum lightning with classical semi-verification can be constructed from two-tier one-shot signatures in a black-box way:
\begin{theorem}
\label{thm:OSStoQL}
If two-tier one-shot signatures exist, then two-tier quantum lightning with classical semi-verification exist.    
\end{theorem}
\begin{proof}[Proof of \cref{thm:OSStoQL}]
Let $(\KeyGen',\StateGen',\Sign,\Ver_0,\Ver_1)$    
be a two-tier one-shot signature. From it, we construct two-tier quantum lightning with classical semi-verification $(\KeyGen,\StateGen,\SemiVer,\FullVer)$ as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to(\sk,\pk):$
    Run $\KeyGen'(1^\secp)\to(\sk',\pk')$.
    Output $\sk\coloneqq \sk'$ and $\pk\coloneqq \pk'$.
    \item 
    $\StateGen(\pk)\to\psi:$
    Run $\StateGen'(\pk)\to\psi'$.
    Output $\psi\coloneqq\psi'$.
    \item 
    $\SemiVer(\pk,\psi)\to\top/\bot:$
    Run $\Sign(\psi,0)\to\sigma_0$.
    Run $\Ver_0(\pk,\sigma_0)$ and output its output.
     \item 
    $\FullVer(\sk,\psi)\to\top/\bot:$
    Run $\Sign(\psi,1)\to\sigma_1$.
    Run $\Ver_1(\sk,\sigma_1)$ and output its output.
\end{itemize}
Both correctness and security are clear.
\end{proof}

